Hearts and towers in stable infinity-categories

We exploit the equivalence between $t$-structures and normal torsion theories on a stable $\infty$-category to show how a few classical topics in the theory of triangulated categories, i.e., the characterization of bounded $t$-structures in terms of their hearts, their associated cohomology functors, semiorthogonal decompositions, and the theory of tiltings, as well as the more recent notion of Bridgeland's slicings, are all particular instances of a single construction, namely, the tower of a morphism associated with a $J$-slicing of a stable $\infty$-category $\mathcal C$, where $J$ is a totally ordered set equipped with a monotone $\mathbb{Z}$-action.

==> files/05-hearts-revised-K.tex <==
%!TEX root=../hearts-revised.tex
\section{Hearts of $J$-slicings.}\label{hearts}
\begin{modifyepigraph}{.9}
\epigraph{I watched a snail crawl along the edge of a straight razor. That's my dream. That's my nightmare. Crawling, slithering, along the edge of a straight razor\dots\ and surviving.
}{Col. W\@. E\@. Kurtz}
\end{modifyepigraph}

Recall the equivalence relation $x\sim y$ if and only if there are integers $a,b \in \Z$ with $a\leq b$ such that $x + a \le y \le x + b$ on a $\Z$-toset $J$ from lemma \refbf{equivalence}.
\begin{lemma}\label{heartability}
The following are equivalent:
\begin{enumerate}[label=$\roman*$)]
\item the  $\Z$-toset $J$ consists of a single equivalence class with respect to the equivalence relation $\sim$; 
\item there exists an interval $I$ in $J$ such that the map $\varphi\colon (n,x)\mapsto x+n$ is an isomorphism of $\Z$-tosets $\Z\times_{\mathrm{lex}}I\xrightarrow{\sim} J$ (where the $\Z$-action on $I$ is the trivial one and the $\Z$-action on $\Z$ is the translation).
\end{enumerate}
\end{lemma}
\begin{proof}
That $(i)$ implies $(ii)$ is an immediate consequence of \refbf{lemma.representatives}. To prove the converse implication notice that since $\varphi$ is surjective every element in $J$ is equivalent to an element in $I$. So we are reduced to show that all elements in $I$ are equivalent each other. Let $x,y\in I$. We can assume $x\leq y$. Since $J$ is totally ordered we have either $y\leq x+1$ or $x+1\leq y$. In the latter case we have $x\leq x+1\leq y$ and so $x+1\in I$, since $I$ is an interval. But then $\varphi(1,x)=\varphi(0,x+1)$ against the hypothesis on $\varphi$. So we are left with $x\leq y\leq x+1$ which implies $x\sim y$.  
\end{proof}
\begin{definition}
Let $J$ be a $\Z$-toset. A \emph{heart} for $J$ is an interval $J^\heart\subseteq J$ such that $\varphi\colon (n,x)\mapsto x+n$ is an isomorphism of $\Z$-tosets $\Z\times_{\mathrm{lex}}J^\heart \xto{\sim} J$.
\end{definition}
\begin{remark}\label{hasaheart}
Of course, not every $\Z$-toset has a heart. It is easy to see that $J$ has an heart if and only if there is a morphism of $\Z$-tosets $\pi_\heart\colon J \to \Z$. An heart of $J$ is given by $\pi_\heart^{-1}(0)$ in this case.
\end{remark}
\begin{remark}
It is immediate from the definition that $J^\heart$ is a heart of $J$ if and only if $J^\heart+n$ is a heart of $J$, for every $n\in \Z$.
\end{remark}
\begin{example}
If $J=\Z$, with the standard $\Z$-toset structure, the hearts of $J$ are the singletons $\{n\}$ with $n\in \Z$. In particular $\{0\}$ is the standard heart of $\Z$, and all the other hearts are shifts of this. If $J=\mathbb{R}$, with the standard $\Z$-toset structure, then the hearts of $J$ are the intervals of the form $[x,x+1)$ and those of the form $(x,x+1]$, with $x\in \mathbb{R}$.
\end{example}

\begin{example}\label{I.has.a.heart}
Let $(J, \leq)$ be a totally ordered $\mathbb{Z}$-poset, and let $\sim$ be the equivalence relation from Lemma \refbf{equivalence}. For every $i\in J$ let $I_i$ be the equivalence class of $i$. This is an interval in $J$, see Example \refbf{class.is.interval}. Moreover, by Lemma \refbf{lemma.representatives}, $I_i$ has a heart precisely when $i$ is not a fixed point of the $\Z$-action.
\end{example}

\begin{lemma}\label{lemma.plus.one}
Let $I\colon \uno \to \O(J)$ be a heart of $J$. Then $I(1)=I(0)+1$, i.e., $U_1=U_0+1$ (equivalently, $L_1=L_0+1$).
\end{lemma}
\begin{proof}
Assume $U_1\nsubseteq U_0+1$. Then there exists an element $x$ in $U_1\cap(L_0+1)$. Since $I$ is a heart, there exists an element $y$ in $I$ and an integer $n$ such that $x=y+n$. If $n\geq 1$ we have $y+n\in U_0+n\subseteq U_0+1$ and so $x\in (U_0+1)\cap (L_0+1)$, which is impossible. If $n\leq 0$ we have $y+n\in L_1+n\subseteq L_1$ and so $x\in L_1\cap U_1$ which again is impossible. Therefore $U_1\subseteq U_0+1$. Now assume $U_0+1\nsubseteq U_1$. Then there exists an element $x\in (U_0+1)\cap L_1$. Let $y=x-1$. Then $y\in U_0\cap (L_1-1)\subseteq U_0\cap L_1=I$. Since $U_0+1\subseteq U_0$ we also have $x\in I$, and so $\varphi(-1,x)=\varphi(0,y)$, which is impossible. Therefore $U_1= U_0+1$.
\end{proof}
\begin{definition}
Let $J^\heart\subseteq J$ be a heart of $J$ and let $\tee\colon \O(J)\to  \ts(\C)$ be a $J$-slicing on a stable $\infty$-category $\C$. The subcategory $\C_{J^\heart}$ of $\C$ will be called a \emph{heart} of the $J$-slicing $\tee$ and will be denoted $\C^\heart$.
\end{definition}
\begin{notat}
We denote the canonical projection to the heart as $\mathcal{H}^\heart\colon \C\to \C^\heart$; see \adef\refbf{def.homology}.
\end{notat}
\begin{example}
We have seen in Example\refbf{ex.Z-is-t} that a  a $\Z$-slicing on a stable $\infty$-category $\C$ is the same thing as the datum of a $t$-structure $\tee=(\C_{<0},\C_{\geq 0})$ on $\C$. The standard heart $\C^\heart=\C_{\{0\}}$ is called the heart of the $t$-structure $\tee$. The projection to the heart is the functor $\mathcal{H}^0$; see Notation \refbf{Hi}.
\end{example}

From \refbf{cor:perPostnikov} we immediately get the following
\begin{proposition}\label{cor.oss.for.Heart.to.t}
Let $\tee=(\C_{<0},\C_{\geq 0})$ be a bounded $t$-structure on a stable $\infty$-category $\C$, and let $\C^\heart=\C_0$ be its standard heart. Then $\tee$ is completely determined by the functors $\mathcal{H}^j\colon \C \to \C^\heart[j]$ (and so by the functor $\mathcal{H}^0$ alone). More precisely, $\C_{\geq 0}$ is the full subcategory of $\C$ on the objects $Y$ such  that $\mathcal{H}^jY=0$ for any $j< 0$, while $\C_{< 0}$ is the full subcategory of $\C$ on those objects $Y$ for which $\mathcal{H}^jY=0$ for any $j\geq 0$.
\end{proposition}


\begin{remark}\label{evocative}
There is a rather evocative pictorial representation of the heart $\C_{[0,1)}$ of an $\mathbb{R}$-slicing, manifestly inspired by \cite{Brid}: if we depict $\C_{<0}$ and $\C_{\geq 0}$ as contiguous half-planes (refer to Figure \refbf{figure:slices})
then the action of the shift functor can be represented as an horizontal shift, and the closure properties of the two classes $\C_{<0}, \C_{\geq 0}$ under positive and negative shifts are a direct consequence of the shape of these areas. With these notations, an object $Z$ is in the heart $\C_{[0,1)}$ if it lies in a ``boundary region'', \ie if it lies in $\C_{\geq 0}$, but $Z[-1]$ lies in $\C_{<0}$.
\begin{center}
\begin{figure}[h]
\begin{tikzpicture}
\filldraw[gray!15] (5,-2) -- (-5,-2) -- (-5,2) -- (5, 2) -- cycle;
\filldraw[gray!40] (.5, -2) -- (0,-2) -- (0,2) -- (.5,2) -- cycle;
\draw[thick] (0,-2) -- (0,2);
\fill (2,1) circle (2pt) node[left] (X) {$X$};
\fill (-1,-1) circle (2pt) node[right] (Y) {$Y$};
\node at (4.5,-1.5) {$\C_{\geq 0}$};
\node at (-4.5,-1.5) {$\C_{<0}$};
\draw[->] (2.2,1) -- (2.8,1);
\draw[->] (-1.2,-1) -- (-1.8,-1);
\fill[xshift=1cm] (2,1) circle (2pt) node[right] (X) {$X[1]$};
\fill[xshift=-1cm] (-1,-1) circle (2pt) node[left] (Y) {$Y[-1]$};
\draw (.25,0.5) circle (2pt) node[right] {$Z$};
\draw (-.75,0.5) circle (2pt) node[left] {$Z[-1]$};
\draw[thick, ->, red] (.05,0.5) to (-.55,0.5);
\draw[->, xshift=-.5cm, yshift=-.5cm] (-5,-2) -- (6,-2) node[below, pos=.9] {\text{shift}};
\end{tikzpicture}
\caption{Heart of an $\mathbb{R}$-slicing}
\label{figure:slices}
\end{figure}
\end{center}
\end{remark}


Let now $J^\heart\subseteq J$ be a heart, and let $\C^\heart=\C_I$ be the corresponding subcategory of $C$, relative to a given $J$-slicing $\tee$. Writing $I$ as $I\colon \uno \to \O(J)$, for any $n\in \Z$ and any $k\geq 0$ we can consider the interval decomposition $I_{\ordered{k}}\colon \ordered{k}\to \O(J)$ defined by setting $I_{\ordered{k}}(j)=I(0)+j+n$ for $0\leq j\leq k$. By Lemma \refbf{lemma.plus.one}, this corresponds to the collection of $n$ contiguous intervals $I+n,I+n+1,\dots,I+n+k-1\subseteq J$. The corresponding subcategories of $\C$ will be $\C^\heart[n]$, $\C^\heart[n+1]$,\dots,$\C^\heart[n+k-1]$.



 The existence and uniqueness of $I_{\ordered{k}}$-weaved factorizations then specializes to the following statement
\begin{proposition}\label{prop.first-tower}
Let $f\colon X\to Y$ be a morphism in $\C$. Then for any integer $n$ and any positive integer $k$ there exists a unique factorization
\[
X \xto{f_{n+k}} Z_{n+k-1} \xto{f_{n+k-1}}Z_{n+k-2}\to\dots\to Z_{n+1} \xto{f_{n}} Z_{n} \xto{f_{n-1}} Y,
\]
of $f$ such that
$\cofib(f_j)\in \C^\heart[j]$ for any $j=n,\dots,n+k-1$,  $\cofib(f_{n-1})\in \C_{L_0}[n]$  and $\cofib(f_{n+k})\in \C_{U_k}[n]=\C_{U_0}[k+n]$.
\end{proposition}
The content of \aprop\refbf{prop.first-tower} becomes more interesting when $\C$ is \emph{bounded} with respect to the $J$-slicing $\tee$ (see \adef\refbf{def.bounded}), as in this case $\cofib(f)$ lies in $\C_{U_0}[n]$ for $n\ll 0$ and in $\C_{L_0}[n]$ for $n\gg0$ . Namely, if $\C$ is $J$-bounded, then $\cofib(f)$ lies in $\C_{\geq i}$ for some $i\in J$. Since $J^\heart$ is a heart, there exists an element $x\in I$ and an integer $n_0$ such that $i=x+n_0$, so that $\cofib(f)\in \C_{\geq x}[n_0]$. As $x\in I$ we have $x\in U_0$ and so $[x,+\infty)\subseteq U_0$ therefore $\cofib(f)\in \C_{U_0}[n_0]$ and so $\cofib(f)\in \C_{U_0}[n]$ for any $n\leq n_0$. Dually one proves the statement for $n\gg0$. 
 As an immediate consequence, by Remark \refbf{rem.trivial-factorizations} we see that in the $J$-bounded case
if $f\colon X\to Y$ is any morphism in $\C$, then  
 the morphisms $0 \to \cofib(f)_{n+k-1}$ and $\cofib(f)_{n} \to \cofib(f)$ in $\rook\Big(\varnobkt{0}{\cofib(f)},I_{\ordered{k}}\Big)$ are isomorphisms for $n\ll 0$ and $k \gg 0$. Since $\rook\Big(\varnobkt{0}{\cofib(f)},I_{\ordered{k}}\Big)$ is the $I_{\ordered{k}}$-weaved factorization of $0\to \cofib(f)$ by Corollary \refbf{cor:perPostnikov}, and since isomorphisms are preserved by pullouts we see that both $X \xto{f_{n+k}} Z_{n+k-1} $ and $Z_{n} \xto{f_{n-1}} Y$ are isomorphisms.
 
 %One notices, as it is obvious, that the class of isomorphisms in $\C$ is closed under transfinite composition 
 \par
 This leads to the following
\begin{proposition}\label{prop.Z.Postnikov}
Let $\C$ be a stable $\infty$-category which is bounded with respect to a given $J$-slicing $\tee$. Let $J^\heart\subseteq J$ be a heart for $J$ and let $\C^\heart$ be the corresponding heart in $\C$.
Then for any morphism $f\colon X\to Y$  in $\C$ there exists an integer $n_0$ and a positive integer $k_0$ such that for any integer $n\leq n_0$ and any positive integer $k$ with $k\geq n_0-n+k_0$ there exists a unique factorization of $f$ 
\[
X \xto{\sim} Z_{n+k-1} \xto{f_{n+k-1}}Z_{n+k-2}\to\dots\to Z_{n+1} \xto{f_{n}} Z_{n} \xto{\sim} Y
\]
such that
$\cofib(f_j)\in \C^\heart[j]$ for any $j=n,\dots,n+k-1$.
\end{proposition}
\begin{remark}\label{oss.Z.Postnikov}
By uniqueness in \aprop\refbf{prop.Z.Postnikov}, one has a well defined $\Z $-factorization
\[
X=\lim(Z_j) \to\cdots \to Z_{j+1} \xto{f_{j}} Z_{j} \xto{f_{j-1}}Z_{j-1}\to \cdots\to \mathrm{colim}(Z_j)=Y
\]
with $j$ ranging over the integers, $\cofib(f_j)\in \C^\heart[j]$ for any $j\in \Z $ and with $f_m$ being an isomorphism for $|j|\gg 0$. We will refer to this factorization as the $\C^\heart$-weaved factorization of $f$. Notice how the boundedness of $\C$ has played an essential role: when $\C$ is not bounded, one still has towers for interval decomposition $I_{\ordered{k}}\colon j\mapsto I(0)+j+n$ for arbitrary $k$ and $n$, but in general they do not stabilize.
\end{remark}
\begin{remark}\label{oss.for.Heart.to.t}
Let $J^\heart\subseteq J$ be a heart, and let $(L,U)$ be the slicing $J^\heart(0)$ of $J$ and $\tee=(\C_U,\C_L)$ be the corresponding $t$-structure on $\C$. By Lemma \refbf{lemma.plus.one} the standard heart of $\tee$ is precisely $\C^\heart$. Moreover,
by Corollaries \refbf{cor:perPostnikov} and \refbf{perPostnikov2}, the $\C^\heart$-weaved factorization 
\[
0=\lim(Y_j) \to\cdots \to Y_{j+1} \xto{f_{j}} Y_{j} \xto{f_{j-1}}Y_{j-1}\to \cdots\to \mathrm{colim}(Y_j)=Y
\]
of an initial morphism $0\to Y$ is such that $\cofib(f_j)=\mathcal{H}^jY$ for any $j\in \Z$. Therefore we see that the $t$-structure $(\C_L,\C_U)$ can be completely read from $\C^\heart$-weaved factorizations: an object $Y$ is in $\C_{U}$ if and only if the $\C^\heart$-weaved factorization of $0\to Y$
satisfies $\cofib(f_j)=0$ for any $j< 0$, while $Y$ is in $\C_{L}$ if and only if  $\cofib(f_j)=0$ for any $j\geq 0$. We are going to use this fact later to characterize hearts of $t$-structures among full subcategories of $\C$.
\end{remark}

\begin{remark}\label{bounded.is.bounded}
The content of Remark \refbf{oss.for.Heart.to.t} can be elegantly expressed in terms of the functoriality of slicings (Remark \refbf{rem.slicing-functor}). Namely, by Remark \refbf{hasaheart}, to give a heart $J^\heart$ of $J$ is equivalent to giving  a $\Z$-equivariant morphism of $\pi_\heart\colon \Z$-tosets $J\to\Z$, and by functoriality this induces a map
\[
\pi_\heart\colon \slicings(J,\C)\to \ts(\C).
\]   
The heart $\C^\heart$ of a $J$-slicing $\tee$ on $\C$ is then the standard heart of the corresponding $t$-structure $\pi_\heart(\tee)$. Moreover, one easily sees that $\tee$ is a bounded $J$-slicing if and only if $\pi_\heart(\tee)$ is a bounded $t$-structure. Indeed, since $\pi_\heart$ is a morphism of tosets, for any $i_1\leq i_2$ in $J$ we have $[i_1,i_2]\subseteq \pi_\heart^{-1}[\pi_\heart(i_1),\pi_\heart(i_2)]$. Vice versa, since  $\pi_\heart$ is $\Z$-equivariant, for every $j\in J$ we have $\pi_\heart(j+n)=\pi_\heart(j)+n$ and so for every $n_1\leq n_2$ in $\Z$ there exist $j_1\leq j_2$ in $J$ such that $\pi_\heart(j_1)< n_1$ and $\pi_\heart(j_2)> n_2$. Let $j\in J$ be such $n_1\leq \pi_\heart(j)\leq n_2$. If $j>j_2$ then we would have $\pi_\heart(j)\geq \pi_\heart(j_2)>n_2$, and so $j\leq j_2$. Similarly $j\geq j_1$ and so $\pi_{\heart}^{-1} [n_1,n_2]\subseteq [j_1,j_2]$.
\end{remark}


\subsection{Abelianity of the heart.}
In the following section we present a proof of the fact that a heart $\C^\heart$ of a $J$-slicing on a stable $\infty$-category $\C$
is an abelian $\infty$-category. 

In other words, $\C^\heart$ is homotopy equivalent to its homotopy category $h\C^\heart$, which is an abelian category; this is the higher-categorical counterpart of a classical result, first proved in \cite[Thm. \textbf{1.3.6}]{BBDPervers}, 
which 
only relies on properties stated in terms of normal torsion theories in a stable $\infty$-category. 
We begin with the following
\begin{definition}[Abelian $\infty$-category]\label{df:abelinfty}
An \emph{abelian $\infty$-category} is a quasicategory $\cate{A}$ such that
\begin{enumerate}[label=$\roman*$)]
\item the hom space $\cate{A}(X,Y)$ is a homotopically discrete infinite loop space for any $X, Y$, \ie, there exists an infinite sequence of $\infty$-groupoids $Z_0, Z_1,Z_2,\dots$, with $Z_0\cong \C(X,Y)$ and homotopy equivalences $Z_i\cong \Omega Z_{i+1}$ for any $i\geq 0$, such that $\pi_n Z_0=0$ for any $n\geq 1$;
\item $\cate{A}$ has a zero object, (homotopy) kernels, cokernels and biproducts;
\item for any morphism $f$ in $\cate{A}$, the natural morphism from the \emph{coimage} of $f$ to the \emph{image} (see \adef\refbf{imcoim}) of $f$ is an equivalence.
\end{enumerate}
\end{definition}
\begin{remark}
Axiom (i) is the homotopically-correct version of $\cate{A}(X,Y)$ being an abelian group. For instance, if the abelian group is $\Z $, then the corresponding homotopy discrete space is the Eilenberg-Mac Lane spectrum $\Z ,K(\Z ,1), K(\Z ,2),\dots$. The homotopy category of such an $\cate{A}$ is an abelian category in the classical sense (note that $\cate{A}(X,Y)$ being homotopically discrete is necessary in order that kernels and cokernels in $\cate{A}$ induce kernels and cokernels in $h\cate{A}$). Moreover, since the hom spaces $\cate{A}(X,Y)$ are homotopically discrete, the natural morphism $\cate{A}\to h\cate{A}$ is actually an equivalence.
\end{remark}

The rest of the section is devoted to the proof of the following result:
\begin{theorem}\label{heart.is.abelian}
Let $\C^\heart$ be a heart of a $J$-slicing $\tee$ on a stable $\infty$-category $\C$. Then $\C^\heart$ is an abelian $\infty$-category.\end{theorem}
\begin{remark}
If $J=\Z$, so that $\tee$ is the datum of a $t$-structure on $\C$, and $\C^\heart=\C_{\{0\}}$ is the standard heart of $\C$, the the  homotopy category $h\C^\heart$ is the abelian category arising as the standard heart of the $t$-structure $h(\tee)$ on the triangulated category $h\C$.
\end{remark}
In what follows, let $I\colon \uno \to \O(J)$ be an interval such that $\C^\heart=\C_I$. The two factorization systems associated with $I$ will be denoted by $(\E_0,\M_0)$ and $(\E_1,\M_1)$, respectively. By Lemma \refbf{lemma.plus.one} we have $\M_1=\M_0[1]$ and $\E_1=\E_0[1]$.
\begin{lemma}
For any $X$ and $Y$ in $\C^\heart$, the hom space $\C^\heart(X,Y)$ is a homotopically discrete infinite loop space.
\end{lemma}
\begin{proof}
Since $\C^\heart$ is a full subcategory of $\C$, we have $\C^\heart(X,Y)=\C(X,Y)$, which is an infinite loop space since $\C$ is a stable $\infty$-category. 

So we are left to prove that $\pi_n\C(X,Y)=0$ for $n\geq 1$. Since $\pi_n\C(X,Y)=\pi_{n-1}\Omega\C(X,Y)=\pi_{n-1}\C(X,Y[-1])$, this is equivalent to showing that 
$\C(X,Y[-1])$ is contractible. Since $X$ and $Y$ are objects in $\C^\heart$, we have $X\in \C_{U_0}$ and $Y[-1]\in \C_{L_1[-1]}=\C_{L_1-1}=\C_{L_0}$. But $\C_{L_0}$ is right object-orthogonal to $\C_{U_0}$, therefore $\C(X,Y[-1])$ is contractible.
\end{proof}

The subcategory $\C^\heart$ inherits the $0$ object and biproducts (in fact, all finite limits) from $\C$, so in order to prove it is is abelian we are left to prove that it has kernels and cokernels, and that the canonical morphism from the coimage to the image is an equivalence.
\begin{lemma}\label{lemma.qua.e.la}
Let $f\colon X\to Y$ be a morphism in $\C^\heart$. Then $\mathrm{fib}(f)$ is in $\C_{L_1}$ and $\cofib(f)$ is in $\C_{U_0}$.
\end{lemma}
\begin{proof}
Since both $X\to 0$ and $Y\to 0$ are in $\M_1$, by the 3-for-2 property also $f$ is in $\M_1$. Since $\M_1$ is closed for pullbacks, $\mathrm{fib}(f)\to 0$ is in $\M_1$ and so $\mathrm{fib}(f)$ is in $\C_{L_1}$. The proof for $\cofib(f)$ is completely dual.
\end{proof}
\begin{definition}
Denote by
\[
% \xymatrix{
% 0\ar[r]^-{\E_0}&\ker(f)\ar[r]^{\M_0}&\fib(f)
% }
\begin{kodi}
\obj (m) {0 & \ker(f) & \fib(f)};
\mor (m-1-1) -> (m-2-1);
\mor (m-2-1) -> (m-3-1);
\end{kodi}
\]
the $(\E_0,\M_0)$-factorization of the morphism $0\to \fib(f)$
and by
\[
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \xymatrix{
% \cofib(f)\ar[r]^{\E_1}&\coker(f)\ar[r]^-{\M_1} &0
% }
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{kodi}
\obj (m) {\cofib(f) & \coker(f) & 0 };
\mor (m-1-1) -> (m-2-1);
\mor (m-2-1) -> (m-3-1);
\end{kodi}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\]
the $(\E_1,\M_1)$-factorization of the morphism $\cofib(f)\to 0$. We call $\ker(f)$ and $\coker(f)$ respectively the \emph{kernel} and the \emph{cokernel} of $f$ in $\C^\heart$.
\end{definition}
\begin{remark}\label{oss.miracle}
Since $\cofib(f)[-1]\cong \fib{f}$ and $(\M_1,\E_1)[-1]=(\M_0,\E_0)$, one can equivalently define $\coker(f)$ by declaring the $(\E_0,\M_0)$-factorization of $\fib(f)\to 0$ to be $\fib(f)\xto{\E_0}\coker(f)[-1]\xto{\M_0} 0$. Similarly, one can define $\ker(f)$ by declaring the $(\E_1,\M_1)$-factorization of $0\to \cofib(f)$ to be $0\xto{\E_1}\ker(f)[1]\xto{\M_1} \cofib(f)$.
By normality of the factorization system we therefore have the homotopy commutative diagram 
\[
\begin{kodi}
\obj{
	0  &|(ker)| \ker(f) &[1cm] |(fib)| \fib(f)\\
	&|(0')| 0 &|(coker)| \coker(f)[-1] & |(0'')| 0 \\
};
\mor 0 {\E_0}:-> ker \M_0:-> fib \E_0:-> coker \M_0:-> 0'';
\mor ker \E_0:-> 0' \M_0:-> coker \M_0:-> 0'';
\end{kodi}
\]
whose square sub-diagram is a homotopy pullout.
\end{remark}
\begin{lemma}
Both $\ker(f)$ and $\coker(f)$ are in $\C^\heart$.
\end{lemma}
\begin{proof}
By construction $\ker(f)$ is in $\C_{U_0}$, so we only need to show that $\ker(f)$ is in $\C_{L_1}$. By definition of $\ker(f)$, we have that $\ker(f)\to \fib(f)$ is in $\M_0$. Since $\M_0[-1]\subseteq \M_0$, we have that also $\ker(f)[-1]\to \fib(f)[-1]$ is in $\M_0$.
By Lemma \refbf{lemma.qua.e.la}, $\fib(f)[-1]\to 0$ is in $\M_1[-1]=\M_0$ and so we find that also $\ker(f)[-1]\to 0$ is in $\M_0$. 
The proof for $\coker(f)$ is perfectly dual.
\end{proof}
By definition of $\ker(f)$ and $\coker(f)$, the defining diagram of $\fib(f)$ and $\cofib(f)$ can be enlarged as
\[
\begin{kodi}
\obj{
0 & |(ker)| \ker(f) & |(fib)| \fib(f) & X & |(01)| 0 \\
& &|(02)| 0 & Y & |(cofib)| \cofib(f) & |(coker)| \coker(f) & |(03)| 0\\	
};
\mor 0 -> ker -> fib -> X -> 01 -> cofib -> coker -> 03;
\mor fib -> 02 -> Y -> cofib;
\mor X f:-> Y;
\mor ker k_f:{bend left=60},-> X; \mor Y c_f:{bend right=60},-> coker;
\end{kodi}
\]
where $k_f$ and $c_f$ are morphisms in $\C^\heart$.
\begin{definition}\label{imcoim}
Let $f\colon X\to Y$ be a morphism in $\C^\heart$. The \emph{image} $\im(f)$ and the \emph{coimage} $\coim(f)$ of $f$ are defined as $\im(f)=\ker(c_f)$ and  $\coim(f)=\coker(k_f)$. 
\end{definition}
The following lemma shows that $\ker(f)$ does indeed have the defining property of a kernel:
\begin{lemma}\label{is.a.kernel}
The homotopy commutative diagram
\[
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \xymatrix{
% \ker(f)\ar[r]^{k_f}\ar[d]&X\ar[d]^{f}\
% 0\ar[r]&Y}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{kodi}
\obj (m) {\ker(f) & X & \0 & Y & \\};
\mor (m-1-1) -> (m-2-1);
\mor (m-1-1) -> (m-1-2);
\mor (m-1-2) -> (m-1-3);
\mor (m-2-1) -> (m-3-1);
\end{kodi}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\]
is a pullback diagram in $\C^\heart$.
\end{lemma}
\begin{proof}
A homotopy commutative diagram 
\[
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \xymatrix{
% K\ar[r]\ar[d]&X\ar[d]^{f}\
% 0\ar[r]&Y}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{kodi}
\obj (m) {K & X & \0 & Y & \\};
\mor (m-1-1) -> (m-2-1);
\mor (m-1-1) -> (m-1-2);
\mor (m-1-2) -> (m-1-3);
\mor (m-2-1) -> (m-3-1);
\end{kodi}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\]
between objects in the heart is in particular a homotopy commutative diagram in $\C$ so it is equivalent to the datum of a morphism $k'\colon K\to \fib(f)$ in $\C$, with $K$ an object in $\C^\heart$. By the orthogonality of $(\E_0,\M_0)$, this is equivalent to a morphism $\tilde{k}\colon K\to\ker(f)$:
\[%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \xymatrix{
% 0\ar[r]\ar[d]_{\E_0}&\ker(f)\ar[d]^{\M_0}\
% K\ar[ru]^{\tilde{k}}\ar[r]_{k'}&\fib(f)
% }
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{kodi}
\obj (m) {0 & \ker(f) & \K & \fib(f) & \\};
\mor (m-1-1) -> (m-2-1);
\mor (m-1-1) -> (m-1-2);
\mor (m-1-2) -> (m-1-3);
\mor (m-2-1) -> (m-3-0);
\mor (m-2-1) -> (m-3-1);
\end{kodi}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%. 
\qedhere 
\]
\end{proof}
There is, obviously, a dual result showing that $\coker(f)$ is indeed a cokernel.
\begin{lemma}
The homotopy commutative diagram
\[
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \xymatrix{
% X\ar[r]\ar[d]_{f}&0\ar[d]\
% Y\ar[r]^-{c_f}&\coker(f)
% }
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{kodi}
\obj (m) {X & 0 & \Y & \coker(f) & \\};
\mor (m-1-1) -> (m-2-1);
\mor (m-1-1) -> (m-1-2);
\mor (m-1-2) -> (m-1-3);
\mor (m-2-1) -> (m-3-1);
\end{kodi}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\]
is a pushout diagram in $\C^\heart$.
\end{lemma}

\begin{proposition}\label{pullout.is.pullout}
A homotopy commutative diagram
\[
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \xymatrix{
% X\ar[r]^{f}\ar[d]&Y\ar[d]_{g}\
% \zero\ar[r]&Z
% }
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{kodi}
\obj (m) {X & Y & \\zero & Z & \\};
\mor (m-1-1) -> (m-2-1);
\mor (m-1-1) -> (m-1-2);
\mor (m-1-2) -> (m-1-3);
\mor (m-2-1) -> (m-3-1);
\end{kodi}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\]
with vertices in $\C^\heart$ is a pullout diagram in $\C^\heart$ if and only if it is a pullout diagram in $\C$. 
\end{proposition}
\begin{proof}
Since $\C^\heart$ is a full subcategory of $\C$ it is clear that if the given diagram is a pullout in $\C$ then it is automatically also a pullout in $\C^\heart$. Conversely, assume the given diagram is a pullout in $\C^\heart$. This means that $X=\ker(g)$ and $Z=\coker(f)$. By definition of $\ker$ and $\coker$ this implies that we have the following homotopy commutative diagram in $\C$ where each square is a pullout (in $\C$):
\[
\begin{kodi}%[training wheels]
\obj{
   |(01)|\zero &[1cm]  X &[1cm]  \fib(g)  &[1cm] Y \\
&  |(02)|\zero &  W & \cofib(f)     \\
&& |(03)|\zero &  Z                 \\
&&&|(04)|\zero.                     \\
};
\mor 01 \E_0:-> X \E_0:-> 02 -> W \E_0:-> 03 -> Z \M_1:-> 04;
\mor X \M_0:-> {fib g} \E_0:-> W -> {cofib f} \E_1:-> Z;
\mor {fib g} -> Y -> {cofib f};
\mor X f:dashed,{bend left},-> Y g:dashed,{bend left=50},-> Z;
\end{kodi}
\]
Here $X\to \zero$ is in $\E_0$ by definition of $\ker(g)$ and by the Sator lemma, and so also $\fib(g)\to W$ is in $\E_0$ since $\E_0$ is closed under pushouts.
The morphism $\cofib(f)\to Z$ is in $\E_1$ by definition of $\coker(f)$. From the pullout diagram in $\C$
\[
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \xymatrix{
% \cofib(f)\ar[r]\ar[d] & \zero\ar[d]\
% Z\ar[r] & W[1]
% }
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{kodi}
\obj (m) {\cofib(f) & \zero & \Z & W[1] & \\};
\mor (m-1-1) -> (m-2-1);
\mor (m-1-1) -> (m-1-2);
\mor (m-1-2) -> (m-1-3);
\mor (m-2-1) -> (m-3-1);
\end{kodi}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\]
 and the fact $\E_1$ is closed under pushouts that follows that $\zero\to W[1]$ is in $\E_1$. Therefore $\zero\to W$ is in $\E_1[-1]=\E_0$ and so $W\to \zero$ is in $\E_0$. This shows that $\fib(g)\to \zero$ is in $\E_0$ and so $X\to \fib(g)$ is an isomorphism. Therefore the given diagram is a pullback in $\C$ and so a pullout in $\C$. 
\end{proof}




\begin{lemma}\label{lemma.titanic}
For $f\colon X\to Y$ a morphism in $\C$, there is a homotopy commutative diagram where all squares are homotopy pullouts:
\[
\begin{kodi}
\obj{
|(ker)| \ker(f) &[1cm] |(fib)| \fib(f) &[1cm] X &[1cm] 0 &[1cm]\\
|(01)| 0 &|(coker-1)| \coker(f)[-1] & |(Z)| Z_f &|(ker1)| \ker(f)[1] &|(02)| 0 \\
& |(03)| 0 & Y & |(cofib)| \cofib(f) & |(coker)| \coker(f) \\
};
\mor ker -> fib -> X -> 0 {{\E_1}}:-> ker1 -> 02 {{\M_1}}:-> coker;
\mor ker {\E_0}:-> 01 -> coker-1 -> Z -> ker1 {{\M_1}}:-> cofib -> coker;
\mor fib {\E_0}:-> coker-1 {\M_0}:-> 03 -> Y -> cofib;
\mor[swap] X {\E_0}:-> Z {{\M_1}}:-> Y;
\mor X f:{near start},dashed,{bend left},-> Y; 
\mor ker k_f:{bend left},-> X; 
\mor[swap] Y c_F:{bend right},-> coker;
\end{kodi}\]
uniquely determining an object $Z_f\in \C^\heart$.
\end{lemma}
\begin{proof}
Define $Z_f$ as the homotopy pullout
\[
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \xymatrix{
% \fib(f)\ar[r]\ar[d]_{\E_0} \pp & X\ar[d]^{\E_0}\
% \coker(f)[-1]\ar[r]& Z_f}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{kodi}
\obj (m) {\fib(f) & X & \\coker(f)[-1] & Z_f & \\};
\mor (m-1-1) -> (m-2-1);
\mor (m-1-1) -> (m-1-2);
\mor (m-1-2) -> (m-1-3);
\mor (m-2-1) -> (m-3-1);
\end{kodi}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\]
Here the vertical arrow on the right is in $\E_0$ since the vertical arrow on the left is in $\E_0$ by definition of $\coker(f)$ (see Remark \refbf{oss.miracle}) and $\E_0$ is preserved by pushouts. Next, paste on the left of this diagram the pullout given by Remark \refbf{oss.miracle} and build the rest of the 
diagram by taking pullbacks or pushouts, recalling that $(\E_0,\M_0)[1]=(\E_1,\M_1)$. Use again Remark \refbf{oss.miracle} and the fact that $\M_1$ is closed under pullbacks to see that $Z_f\to Y$ is in $\M_1$. 
Finally, we have 
\[
0\xto{\E_0} X\xto{\E_0} Z_f\xto{\M_1} Y\xto{\M_1} 0,
\]
and so $Z_f$ is in $\C^\heart$.
\end{proof}
\begin{proposition}\label{im.iso.coim}
There is an isomorphism $\im (f)\cong\coim (f)$.\end{proposition}
\begin{proof}
By definition, $\im(f)$ and $\coim(f)$ are defined by the factorizations
\[
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \xymatrix{
% 0\ar[r]^-{\E_0}&\im(f)\ar[r]^{\M_0}&\fib(c_f)
% }
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{kodi}
\obj (m) {0 & \im(f) & \fib(c_f) & \\};
\mor (m-1-1) -> (m-2-1);
\mor (m-1-2) -> (m-2-2);
\end{kodi}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\]
and
\[
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \xymatrix{
% \cofib(k_f)\ar[r]^{\E_1}&\coim(f)\ar[r]^-{\M_1} &0
% }
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{kodi}
\obj (m) {\cofib(k_f) & \coim(f) & 0 & \\};
\mor (m-1-1) -> (m-2-1);
\mor (m-1-2) -> (m-2-2);
\end{kodi}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\]
The diagram in Lemma \refbf{lemma.titanic} shows that we have $\fib(c_f)=Z_f=\cofib(k_f)$. Therefore, 
what we need to exhibit are the $(\E_0,\M_0)$ factorizations of $0\to Z_f$ and the $(\E_1,\M_1)$ factorization of $Z_f\to 0$. Since $Z_f$ is an object in $\C^\heart$, these are
\[
0\xrightarrow{\E_0}Z_f\xrightarrow{\mathrm{id}_{Z_f}}Z_f
\]
and 
\[
Z_f\xrightarrow{\mathrm{id}_{Z_f}}Z_f\xrightarrow{\M_1}0,
\]
respectively, thus giving $\im(f)\cong Z_f\cong \coim(f)$.
\end{proof}

\subsection{Abelian subcategories as hearts.}
By the results in the previous section and by Corollary \refbf{cor.oss.for.Heart.to.t} we see that hearts of bounded $t$-structures are very peculiar subcategories of a stable $\infty$-category $\C$: they are abelian and every morphism in $\C$ admits a unique $\C^\heart$-weaved factorization. As we are going to show, these two properties precisely characterize hearts among full subcategories of $\C$.
\begin{definition}
Let $f\colon X\to Y$ be a morphism in $\C$, and let $\cA$ be an abelian $\infty$-subcategory of $\C$. An $\cA$-weaved factorization of $f$ is a factorization
\[
X=\lim(Z_j) \to\cdots \to Z_{j+1} \xto{f_{j}} Z_{j} \xto{f_{j-1}}Z_{j-1}\to \cdots\to \mathrm{colim}(Z_j)=Y
\]
with $j$ ranging over the integers, $\cofib(f_j)\in \cA[j]$ for any $j\in \Z $ and with $f_m$ being an isomorphism for $|j|\gg 0$.
\end{definition}
\begin{proposition}
Let $\cA$ be an abelian full subcategory of a stable $\infty$-category $\C$, such that any morphism $f\colon X\to Y$  in $\C$ has an $\cA$-weaved factorization. Then the collection of subcategories $\{\cA[n]\}_{n\in \Z}$ is a Bridgeland $\Z$-slicing of $\C$.
\end{proposition}
\begin{proof} Looking at \adef\refbf{def.bridgeland-slicing}, the only thing we need to prove is that $\cA[n_1]\orth\cA[n_2]$ for $n_1>n_2$. Let $X\in \cA[n_1]$ and $Y\in\cA[n_2]$. Then $X=Z_1[n]$ and $Y=Z_2[n_2]$ for suitable $Z_1,Z_2\in \cA$ and so 
\begin{align*}
\C(X,Y)&=\C(Z_1[n_1],Z_2[n_2])\cong  \C(Z_1,Z_2[n_2-n_1])\\
&\cong \Omega^{n_1-n_2}\C(Z_1,Z_2)=\Omega^{n_1-n_2}\cA(Z_1,Z_2),
\end{align*}
where in the last equality we used the fact that $\cA$ is full. Since $n_1-n_2>0$, the space $\Omega^{n_1-n_2}\cA(Z_1,Z_2)$ is contractible by definition of abelian $\infty$-category.
\end{proof}


From proposition \refbf{b-is-discrete} and remark \refbf{rem:b-is-discrete} we then immediately have the following converse of Corollary \refbf{cor.oss.for.Heart.to.t}.
\begin{proposition}\label{to.be.repeated.verbatim}
Let $\cA$ be an abelian full subcategory of a stable $\infty$-category $\C$, such that any morphism in $\C$ has a $\cA$-weaved factorization, and let
$\mathcal{H}^n_B\colon \C\to \cA[n]$ be the functors given by taking the cofibers of the $n$-th morphism in the $\cA$-weaved factorization of the initial morphisms. 
 Let
$\C_{\cA,\geq 0}$ be the full subcategory of $\C$ on those objects $X$ such that $\mathcal{H}^j_B(X)=0$ for any $j< 0$, and let $\C_{\cA,< 0}$ be the full subcategory of $\C$ on those objects $X$ such that $\mathcal{H}^j_B(X)=0$ for any $j\geq 0$. Then $\mathfrak{t}_{\cA}=(\C_{\cA,\geq 0}, \C_{\cA,<0})$ is a $t$-structure on $\C$, the stable $\infty$-category $\C$ is bounded with respect to $\mathfrak{t}_{\cA}$, and the standard heart of $\mathfrak{t}_{\cA}$ is (equivalent to) $\cA$.
\end{proposition}
\begin{proof}
The only thing left to prove is that the standard heart of  $\mathfrak{t}_\cA$ is $\cA$. To see this notice that an object $Y$ lies in $\C^\heart=\C_{\cA,\geq 0}\cap \C_{\cA,<1}$ if and only if the $\cA$-weaved factorization
\[
0 =\lim(Y_j)\to\cdots \to Y_{j+1} \xrightarrow{f_{j}} Y_{j} \xrightarrow{f_{j-1}}Y_{j-1}\to \cdots\to \mathrm{colim}(Y_j)=Y
\]
of its initial morphism has $\mathrm{cofib}(f_j)=0$ for every $j\neq0$, and so it is of the form
\[
\cdots 0 \to 0\to \cdots \to 0\xrightarrow{f_{0}} Y \xrightarrow{\mathrm{id}_Y}Y\xrightarrow{\mathrm{id}_Y} \cdots\xrightarrow{\mathrm{id}_Y}Y\xrightarrow{\mathrm{id}_Y}\cdots,\] 
with $Y=\mathrm{cofib}(f_0)\in \cA$.
\end{proof}




==> kodi.tex <==
\input tikz.tex
\usetikzlibrary{kodi}
\let\kodi\kDRammaOpen
\let\endkodi\kDRammaShut
\endinput


==> t-kodi.tex <==
\writestatus{loading}{ConTeXt User Module / koDi}
\startmodule[kodi]
\usemodule[tikz]
\usetikzlibrary[kodi]
\let\startkodi\kDRammaOpen
\let\stopkodi\kDRammaShut
\stopmodule
\endinput


==> tikzlibrarykodi.bapto.code.tex <==
% βάπτω • (báptō)
%   1. I dip, submerge
%   2. I dye, colour
%   3. I baptise

% Bapto is a node labeling mechanism.
% It allows non-invasive relabeling and preprocessing.

% ,-- input           input hook
% `-> controller --.  the controller conditionally
% ,---[overwrite]--'    (depending upon the given overwriting behaviour)
% `-> trigger -----.    calls the trigger
% ,--- ??? <-------'  either short the keys or do preprocessing here
% `-> dispatcher --.  the dispatcher conditionally
% ,---[overwrite]--|    (depending upon the given overwriting behaviour)
% `-> (name|alias) |    assigns the label
%     output <-----'  output hook

%==[ input ]====================================================================

\pgfqkeys{/bapto/input}{
  .forward to=/bapto/controller
}

%==[ controller/dispatcher ]====================================================

\pgfqkeys{/bapto/overwrite}{.is choice,
  false/.style={/bapto/controller/.code={\def\kDTmp{##1}\ifx\kDTmp\empty\else
                                         \tikz@fig@name\ifx\tikz@fig@name\empty
                                         \pgfqkeys{/bapto}{trigger={##1}}\fi\fi},
                /bapto/dispatcher/.code={\pgfqkeys{/tikz}{name=##1}%
                                         \pgfqkeys{/bapto}{output=##1}}},
  alias/.style={/bapto/controller/.code={\def\kDTmp{##1}\ifx\kDTmp\empty\else
                                         \pgfqkeys{/bapto}{trigger={##1}}\fi},
                /bapto/dispatcher/.code={\pgfqkeys{/tikz}{alias=##1}%
                                         \pgfqkeys{/bapto}{output=##1}}},
  true/.style= {/bapto/controller/.code={\def\kDTmp{##1}\ifx\kDTmp\empty\else
                                         \pgfqkeys{/bapto}{trigger={##1}}\fi},
                /bapto/dispatcher/.code={\pgfqkeys{/tikz}{name=##1}%
                                         \pgfqkeys{/bapto}{output=##1}}},
  false, % default is no name overwriting and no aliasing
}

%==[ output ]===================================================================

\pgfqkeys{/bapto/output}{
  .code={}
}


==> tikzlibrarykodi.code.tex <==
% koDi stands for kommutative Diagramme für *TEX*.

%==[ dependencies graph ]=======================================================

% NOTE: arrow notation means targets require sources.

%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~%
%                                %  TikZ/pgf standard libraries
%      calc ------------------.  %
%      matrix -------------.  |  %
%                          |  |  %
%~~~~~~~~~~~~~~~~~~~~~~~~~~|~~|~~%
%                          |  |  %  koDi volatile layer: TikZ bugfixes
%      kodi.diorthono      |  |  %
%                          |  |  %
%~~~~~~~~~~~~~~~~~~~~~~~~~~|~~|~~%
%                          |  |  %  koDi inner layer: base infrastructure
%  ,-> kodi.ektropi ----.  |  |  %
%  |   kodi.bapto ------|  |  |  %
%  |   kodi.katharizo --|  |  |  %
%  `-- kodi.koinos --.  |  |  |  %
%  ,---'             |  |  |  |  %
%~~|~~~~~~~~~~~~~~~~~|~~|~~|~~|~~%
%  |                 |  |  |  |  %  koDi middle layer: custom parsers
%  |-- kodi.mitra <--+--|--'  |  %
%  |-- kodi.ozos <---|  |     |  %
%  |-- kodi.velos <--'  |     |  %
%  |                    |     |  %
%~~|~~~~~~~~~~~~~~~~~~~~|~~~~~|~~%
%  |                    |     |  %  koDi outer layer: user interface
%  `-> kodi.ramma <-----'     |  %
%      kodi.mandyas <---------'  %  TODO: does mandyas depend upon ramma?
%                                %
%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~%

% Given the graph above, these suffice to encompass koDi:

\usetikzlibrary[kodi.diorthono]
\usetikzlibrary[kodi.ramma]
\usetikzlibrary[kodi.mandyas]


==> tikzlibrarykodi.diorthono.code.tex <==
% διορθώνω • (diorthóno)
%   1. I correct
%   2. I mend
%   3. I repair

% Diorthono is a collection of bugfixes.

% Save catcode of @ to restore it at EOF.
\edef\kDAct{\catcode`@=\the\catcode`@\relax}
\catcode`@=11\relax

% The following code patches \pgfpathcurvebetweentime.
% See http://tex.stackexchange.com/a/271024/82186 for reference.
% Original fix by Mark Wibrow.
\def\pgf@@pathcurvebetweentime#1#2#3#4#5#6{%
  \pgfmathparse{#1}%
  \let\pgf@time@s=\pgfmathresult%
  \pgfmathparse{#2}%
  \let\pgf@time@t=\pgfmathresult%
  \ifdim\pgf@time@s pt>\pgf@time@t pt\relax%
    \pgfmathsetmacro\pgf@time@s{1-#1}%
    \pgfmathsetmacro\pgf@time@t{1-#2}%
    \pgf@@@pathcurvebetweentime{#6}{#5}{#4}{#3}%
  \else%
    \pgf@@@pathcurvebetweentime{#3}{#4}{#5}{#6}%
  \fi%
}
\def\pgf@@@pathcurvebetweentime#1#2#3#4{%
\begingroup%
  % Get the curve Q from curve P for time 0 to t
  \pgfextract@process\Pa{#1}%
  \pgfextract@process\Pb{#2}%
  \pgfextract@process\Pc{#3}%
  \pgfextract@process\Pd{#4}%
  % Qa = Pa
  \pgfextract@process\Qa{\Pa}%
  % Qb = Pa + t*(Pb-Pa).
  \pgfextract@process\Qb{%
    \pgfpointadd{\Pa}{\pgfpointscale{\pgf@time@t}{\pgfpointdiff{\Pa}{\Pb}}}%
  }%
  % Qc = Qb + t*((Pb + t*(Pc-Pb)) - Qb)
  \pgfextract@process\Qc{%
    \pgfpointadd{\Qb}{\pgfpointscale{\pgf@time@t}{\pgfpointdiff{\Qb}{\pgfpointadd{\Pb}{\pgfpointscale{\pgf@time@t}{\pgfpointdiff{\Pb}{\Pc}}}}}}%
  }%
  % Qd = (1-t)^3*Pa + 3*t(1-t)^2*Pb + 3*t^2(1-t)*Pc + t^3*Pd.
  \pgfextract@process\Qd{\pgfpointcurveattime{\pgf@time@t}{\Pa}{\Pb}{\Pc}{\Pd}}% 
  %
  % Now get the curve R from the reversed curve Q for time 0 to 1-s/t
  \pgfmathdivide@{\pgf@time@s}{\pgf@time@t}%
  \pgfmathadd@{-\pgfmathresult}{1.0}%
  \let\pgf@time@s=\pgfmathresult%
  % Rd = Qd
  \pgfextract@process\Rd{\Qd}%
  % Rc = Qd + s*(Qc-Qd).
  \pgfextract@process\Rc{%
    \pgfpointadd{\Qd}{\pgfpointscale{\pgf@time@s}{\pgfpointdiff{\Qd}{\Qc}}}%
  }%
  % Rb = Rc + s*((Qc + s*(Qb-Qc)) - Rc)
  \pgfextract@process\Rb{%
    \pgfpointadd{\Rc}{\pgfpointscale{\pgf@time@s}{\pgfpointdiff{\Rc}{\pgfpointadd{\Qc}{\pgfpointscale{\pgf@time@s}{\pgfpointdiff{\Qc}{\Qb}}}}}}%
  }%
  % Ra = (1-s)^3*Qd + 3*s(1-s)^2*Qc + 3*s^2(1-s)*Qb + s^3*Qa.
  \pgfextract@process\Ra{\pgfpointcurveattime{\pgf@time@s}{\Qd}{\Qc}{\Qb}{\Qa}}% 
  \ifpgf@ignoremoveto\else\pgfpathmoveto{\Ra}\fi%
  \pgfpathcurveto{\Rb}{\Rc}{\Rd}%
\endgroup%
}

% Restore catcode of @.
\kDAct


==> tikzlibrarykodi.ektropi.code.tex <==
% εκτροπή • (ektropí)
%   1. diversion
%   2. deflection
%   3. aberration

% Ektropi is a mechanism to hijack the /tikz/.unknown handler.
% It allows the addition of maximum priority paths in the key finding algorithm.
% The diversions are globally scoped, cumulative and removable.

\usetikzlibrary{kodi.koinos}

\kDStoreCatcodeOf @
\catcode`@=11

%==[ handler restoring procedure ]==============================================

% The default handler's code is backed up as a token list at load time.
% NOTE: this has strong implications on loading order!

\newtoks\kDEktropiDefaultToksBackup

\expandafter\expandafter
\expandafter\kDEktropiDefaultToksBackup
\expandafter\expandafter
\expandafter{\csname pgfk@/tikz/.unknown/.@body\endcsname}

\def\kDEktropiRestore{
  % Restore handler body.
  \def\kDAct{\pgfkeyssetvalue{/tikz/.unknown/.@body}}
  \expandafter\kDAct\expandafter{\the\kDEktropiDefaultToksBackup}
  % Restore handler macro.
  % NOTE: #s are doubled since we're inside \kDAct helper.
  \def\kDAct{\long\def\kDAct####1\pgfeov}
  \expandafter\kDAct\expandafter{\the\kDEktropiDefaultToksBackup}
  \pgfkeyslet{/tikz/.unknown/.@cmd}\kDAct
}

% This key is the user interface. Self explanatory.
\pgfkeys{/ektropi/restore/.code={\kDEktropiRestore}}

%==[ handler hacking procedure ]================================================

% This key is the user interface. It wraps the /tikz/.unknown handler code
% with a conditional that executes it only if the unknown key retrieval
% fails inside the path passed to /ektropi/add.
\pgfkeys{/ektropi/add/.style={
  /tikz/.unknown/.add code=
    {
      \let\tikz@key\pgfkeyscurrentname
      \pgfkeys{#1/\tikz@key/.try={##1}}
      \ifpgfkeyssuccess\else
    }{
      \fi
    }
  }
}

\kDRestoreCatcodeOf @


==> tikzlibrarykodi.katharizo.code.tex <==
% καθαρίζω • (katharízo)
%   1. clean, wash
%   2. peel, descale
%   3. (slang) kill

% Katharizo is a detokenization/sanitation mechanism.
% It produces "safe" strings from tokens.

% ,-- input          input hook
% `-> expander ---.  performs expansion according to
% ,---[expand]----'    macro expansion configuration
% `-> expanded ---.  pre-sanitation hook
% ,-- sanitizer <-'  performs detokenization and sanitation according to
% `---[replace]---.    character replacement configuration
% ,-- sanitized <-'  pre-output hook
% `-> output         output hook

%==[ input stage ]==============================================================

\pgfqkeys{/katharizo/input}{
  .forward to=/katharizo/expander
}

%==[ expansion stage ]==========================================================

\pgfqkeys{/katharizo/expand}{.is choice,
  once/.style={/katharizo/expander/.style={/katharizo/expanded/.expand once={##1}}},
  full/.style={/katharizo/expander/.style={/katharizo/expanded/.expanded={##1}}},
  none/.style={/katharizo/expander/.style={/katharizo/expanded={##1}}},
  none % default is no expansion
}

\pgfqkeys{/katharizo/expanded}{
  .forward to=/katharizo/sanitizer
}

%==[ sanitation stage ]=========================================================

\pgfqkeys{/katharizo}{
  replace charcode/.code args={#1 with #2}{%
    % TODO: would a \string be of any use? or at least a stringification?
    \pgfkeys{/katharizo/replacements/characters/#1/.initial={#2}}%
  },
  remove charcode/.style={/katharizo/replace charcode={{#1} with {}}},
  remove charcodes/.style args={#1}{%
    /katharizo/remove charcodes loop={#1 \kD},
  },
  remove charcodes loop/.code args={#1 #2\kD}{%
    % \message{|||#1|#2|||}
    \ifx\relax#1\else\pgfkeys{/katharizo/remove charcode={#1}}\fi
    \ifx\relax#2\else\pgfkeys{/katharizo/remove charcodes loop={#2\kD}}\fi
  },
  replace character/.code args={#1 with #2}{%
    \edef\kDFoo{\number`#1}% TODO: can I inline this?
    % TODO: would a \string be of any use? or at least a stringification?
    \pgfkeys{/katharizo/replacements/characters/\kDFoo/.initial={#2}}%
  },
  remove character/.style={/katharizo/replace character={{#1} with {}}},
  remove characters/.code args={#1#2}{%
    \ifx\relax#1\else\pgfkeys{/katharizo/remove character={#1}}\fi
    \ifx\relax#2\else\pgfkeys{/katharizo/remove characters={#2}}\fi
  },
  remove characters={(),.:},
  remove charcode=92,% \ backslash
}

\pgfqkeys{/katharizo}{
  sanitizer/.code={
    % TODO: token replacement routine? Would that be useful?
    \kDKatharizoStringify#1\kD
    \expandafter\kDKatharizoSanitize\the\kDKatharizoStringified\kD
    \pgfkeysalso{/katharizo/sanitized/.expanded=\the\kDKatharizoSanitized}
    % \message{^^J:::\the\kDKatharizoSanitized:::^^J}
  }
}

\pgfqkeys{/katharizo/sanitized}{
  .forward to=/katharizo/output
}

%==[ output stage ]=============================================================

% NOTE: this must be defined/hooked before calling input
\pgfqkeys{/katharizo/output}{
  .code={}
}

\newtoks\kDKatharizoStringified

\def\kDKatharizoStringify#1\kD{
  \def\kDFoo{#1}
  \edef\kDFoo{\meaning\kDFoo}
  \def\kDAct##1:->##2\kD{##2}
  \edef\kDFoo{\expandafter\kDAct\kDFoo\kD}
  \kDKatharizoStringified\expandafter{\kDFoo}
}

\newtoks\kDKatharizoSanitized

\def\kDKatharizoSanitize#1\kD{
  \pgfkeysifdefined{/katharizo/replacements/characters/32}%
    {\edef\kDKatharizoSSpace{\pgfkeysvalueof{/katharizo/replacements/characters/32}}}%
    {\edef\kDKatharizoSSpace{\space}}%
  \def\kDKatharizoSAppendSpace
    {\edef\kDAct{\noexpand\kDKatharizoSanitized={\the\kDKatharizoSanitized\kDKatharizoSSpace}}\kDAct}
  \kDKatharizoSanitized={}
  \kDKatharizoSString#1 \kD}% NOTE: the whitespace is a mandatory string terminator

\def\kDKatharizoSString#1 #2\kD{%
  \ifx\relax#1\else                       % if string head word is not empty
    \kDKatharizoSWord#1\kD                % parse string head word
    \if#2\space\else                      % if string tail is not the space terminator
      \ifx\relax#2\else                   %   if string tail is not empty
        \kDKatharizoSAppendSpace\fi\fi\fi %     append space substitute to output
  \ifx\relax#2\else                       % if string tail is not empty
    \kDKatharizoSString#2\kD\fi}          %   recurse on string tail

\def\kDKatharizoSWord#1#2\kD{%
  \kDKatharizoSCharacter#1\kD   % parse word head character
  \ifx\relax#2\else             % if word tail is not empty
    \kDKatharizoSWord#2\kD\fi}  %   recurse on word tail

\def\kDKatharizoSCharacter#1\kD{%
  \pgfkeysifdefined{/katharizo/replacements/characters/\number`#1}%
    {\edef\kDFoo{\pgfkeysvalueof{/katharizo/replacements/characters/\number`#1}}}%
    {\edef\kDFoo{#1}}%
  \edef\kDAct{\noexpand\kDKatharizoSanitized={\the\kDKatharizoSanitized\kDFoo}}%
  \kDAct}


==> tikzlibrarykodi.koinos.code.tex <==
% κοινός • (koinós)
%   1. shared
%   2. common
%   3. public

% Koinos implements or aliases commonplace macros.

%==[ catcode manipulation ]=====================================================

\newcount\kDEscapecharCounter

\def\kDEscapecharDisable{\kDEscapecharCounter\escapechar \escapechar=-1}
\def\kDEscapecharEnable{\escapechar\kDEscapecharCounter}

\def\kDStoreCatcodeOf#1%
  {\kDEscapecharDisable
   \expandafter\edef\csname kDRestoreCatcodeOf\string#1\endcsname{\catcode`\string#1=\the\catcode\expandafter`\string#1}%
   % NOTE: setting a default catcode is disabled; might come in handy someday, though.
   % \catcode\expandafter`\string#1=12\relax
   \kDEscapecharEnable}

\def\kDRestoreCatcodeOf#1%
  {\kDEscapecharDisable
   \csname kDRestoreCatcodeOf\string#1\endcsname
   \kDEscapecharEnable}

%==[ forward checks and gobbling ]==============================================

% This macro is the blank space token.
\bgroup
\def\:{\global\let\kDBlankSpace= }\:
\egroup

% Save catcode of @ to restore it later.
\kDStoreCatcodeOf @
\catcode`@=11\relax

% The next two macros both implement token gobbling.

% This "hard" version gobbles any token, ignoring whitespace.
\let\kDGobbleHardTok\pgfutil@gobble

% This "soft" version gobbles only whitespace.
% NOTE: this is just the identity macro. Fun fact.
\def\kDGobbleSoftTok#1{#1}

% The next two macros both implement the following logical condition:
%   if next token is #1 then #2 else #3

% This "hard" version ignores whitespace.
\let\kDIfNextHardCh\pgfutil@ifnextchar

% This "soft" version does not ignore whitespace.
\long\def\kDIfNextSoftCh#1#2#3{%
  \let\kDINCToken= #1% <- MEMO: this space is crucial
  \def\kDINCTrue{#2}\def\kDINCFalse{#3}%
  \futurelet\kDINCTok\kDINC}

\def\kDINC{\ifx\kDINCTok\kDINCToken\let\kDINCFalse\kDINCTrue\fi\kDINCFalse}

% Restore catcode of @.
\kDRestoreCatcodeOf @

%==[ token lists parsing and manipulation ]=====================================

% This macro appends token list #1 to token list #2.
\def\kDAppend#1#2{\edef\kDAct{\noexpand#2={\the#2\the#1}}\kDAct}

% This macro tokenizes the stream into \kDOptTok
% until a group preceeding a ';' character is found;
% then it puts the group into \kDGrpTok and gobbles the ';'.
\def\kDFetchOptAndGrpThen#1%
  {\kDOptTok={}\kDGrpTok={}\kDFetchTilGrpThen{#1}}
  
\newtoks\kDOptTok
\newtoks\kDGrpTok

\def\kDFetchGrpThen#1#2{%
  \def\kDExit{#1}%
  \def\kDLoop{\kDFetchTilGrpThen{#1}}%
  \kDTmpTok={{#2}}%
  \kDIfNextHardCh;
    {\kDGrpTok\the\kDTmpTok\expandafter\kDExit\kDGobbleHardTok}
    {\kDAppend\kDTmpTok\kDOptTok\kDLoop}}

\newtoks\kDTmpTok

\def\kDFetchTilGrpThen#1#2#{%
  \kDTmpTok={#2}%
  \kDAppend\kDTmpTok\kDOptTok
  \kDFetchGrpThen{#1}}

% This macro removes trailing whitespace from token list #1.
\def\kDTrimTrailingSpace#1{%
  \kDDetectTrailingSpace#1
  \ifkDDTSHasTrail
    \def\kDRTS##1 \kD{#1={##1}}%
    \edef\kDRTSAct{\noexpand\kDRTS\the#1\noexpand\kD}
    \kDRTSAct
  \fi}

\def\kDDetectTrailingSpace#1{%
  \kDDTSPrevSpacefalse
  \edef\kDAct{\noexpand\kDDTSGob\the#1\noexpand\kD}%
  \kDAct}

\newif\ifkDDTSHasTrail

\def\kDDTSGob%
  {\kDIfNextSoftCh\kD
    {\message{A}\ifkDDTSPrevSpace\kDDTSHasTrailtrue\else\kDDTSHasTrailfalse\fi\kDGobbleHardTok}
    {\message{B}\kDIfNextSoftCh\kDBlankSpace
      {\message{Y}\kDDTSPrevSpacetrue\expandafter\kDDTSGob\kDGobbleSoftTok}
      {\message{N}\kDDTSPrevSpacefalse\expandafter\kDDTSGob\kDGobbleHardTok}}}

\newif\ifkDDTSPrevSpace

% This macro removes leading whitespace from token list #1.
\def\kDTrimLeadingSpace#1{%
  \def\kDAct##1\kD{#1={##1}}%
  \expandafter\kDGobbleSpaceThen
  \expandafter\kDAct\the#1\kD}

\def\kDGobbleSpaceThen#1%
  {\kDIfNextHardCh\bgroup
    {\kDGSGroupThen#1}
    {\kDGSOtherThen#1}}

\def\kDGSGroupThen#1#2{#1{#2}}

\def\kDGSOtherThen#1#2{#1#2}

%==[ environment checks ]=======================================================

\newif\ifConTeXt
% Trick stolen from iftex. The second line is expanded inside the group so
% the global scope isn't polluted by \csname defining the token.
\begingroup\expandafter\expandafter\expandafter\endgroup\expandafter
  \ifx\csname starttext\endcsname\relax\ConTeXtfalse\else\ConTeXttrue\fi

%==[ dumping, debugging and testing ]===========================================

% macros for dumping, debugging and testing
% TODO: not sure I want to depend on these being in the sourcecode instead of
%   some external package integrated with a TeX unit testing suite.
%   I'll work in that direction.

\newif\ifkDDumping
\kDDumpingfalse

\newwrite\kDDumpFile

\def\kDDumpOpen%
{\ifkDDumping\immediate\openout\kDDumpFile=\jobname.yml\fi}

\def\kDDump#1%
{\ifkDDumping\immediate\write\kDDumpFile{#1}\fi}

\def\kDDumpClose%
{\ifkDDumping\closeout\kDDumpFile\fi}


==> tikzlibrarykodi.mandyas.code.tex <==
% μανδύας • (mandýas)
%   1. cloak
%   2. mantle
%   3. dolman

% Mandias defines the aesthetics aspect of the user level functionality,
% together with some baseline configuration.

\usetikzlibrary[calc]

% \usetikzlibrary[decorations.pathreplacing]
% \usetikzlibrary{decorations.pathmorphing}
% \usetikzlibrary[decorations.markings]
% \usetikzlibrary[arrows.meta]

\pgfqkeys{/kD}{
%==[ universal styles ]=========================================================
  every diagram/.append style={},
  every layout/.append style={
    /kD/every object/.append style={shape=kD baseline centered rectangle},
    square,
  },
  every object/.append style={},
  every arrow/.append style={
    >=stealth,
  },
  every label/.append style={
    auto,
    inner sep=0.5ex,
    font=\everymath\expandafter{\the\everymath\scriptstyle}
  },
%==[ arrow styles ]=============================================================
  /kD/arrows/.cd,
    crossing over/clearance/.initial=0.5ex,
    crossing over/color/.initial=white,
    crossing over/.style={
      /tikz/preaction={
        -,
        draw=\pgfkeysvalueof{/kD/arrows/crossing over/color},
        line width=\pgfkeysvalueof{/kD/arrows/crossing over/clearance},
      },
    },
    shove/.style={
      /tikz/transform canvas={
        /tikz/shift={($(\tikztostart)!#1!-90:(\tikztotarget)-(\tikztostart)$)}
      }
    },
    slide/.style={
      /tikz/transform canvas={
        /tikz/shift={($(\tikztostart)!#1!0:(\tikztotarget)-(\tikztostart)$)}
      }
    },
%==[ label styles ]=============================================================
  /kD/labels/.cd,
    mid/.style={
      /tikz/fill=white,
      /tikz/shape=circle,
      /tikz/anchor=center,
      /tikz/inner sep=.25ex
    },
%=[ objects styles ]============================================================
  /kD/objects/.cd,
    % TODO: reflect on these styles
    % rectangular/.style 2 args={
    %   /tikz/node distance=#2 and #1
    % },
    % square/.style={
    %   /kD/objects/rectangular={#1}{#1}
    % },
    % golden/.style={
    %   /kD/objects/rectangular={#1}{0.618*#1}
    % },
    % % comb/.style={
    % %   /kD/objects/rectangular={#1}{sqrt(3/4)*#1},
    % % },
    % % comb/.default=4em,
    % square/.default=4em,
    % golden/.default=4em,
%=[ lattice styles ]============================================================
  /kD/layouts/.cd,
    rectangular/.style 2 args={
      /tikz/column sep={#1,between origins},
      /tikz/row sep={#2,between origins},
    },
    square/.style={
      /kD/layouts/rectangular={#1}{#1}
    },
    golden/.style={
      /kD/layouts/rectangular={#1}{0.618*#1}
    },
    comb/.code args={#1step #2 angle #3}{
      % TODO: write better option parser
      \if\relax#1\pgfkeys{/kD/layouts/horizontal comb=step #2 angle #3}
      \else\pgfkeys{/kD/layouts/#1comb=step #2 angle #3}\fi
    },
    horizontal comb/.style args={step #1 angle #2}{
      /kD/layouts/rectangular={#1}{tan(#2)*#1*0.5},
      /tikz/every odd row/.append style={/tikz/xshift=(#1)*0.5}
    },
    vertical comb/.style args={step #1 angle #2}{
      /kD/layouts/rectangular={tan(#2)*#1*0.5}{#1},
      /tikz/every odd column/.append style={/tikz/yshift=-1*(#1)*0.5}
    },
    comb/.default=step 4.5em angle 60,
    horizontal comb/.default=step 4.5em angle 60,
    vertical comb/.default=step 4.5em angle 60,
    square/.default=4.5em,
    golden/.default=4.5em,
%=[ diagram styles ]============================================================
  /kD/diagrams/.cd,
    grid/.style 2 args={
      /tikz/x={#1},
      /tikz/y={#2},
      /tikz/on grid
    },
    metric/.style 2 args={
      % NOTE: {1 and 1}{1} is infty-norm, unit circle is unit square
      % NOTE: {2}{0.5} is 1-norm, circle of radius 2 is rhombus circumscribing base hexagon
      /tikz/node distance={#1},
      % TODO: implement control to allow for explicit units on single factor specs
      /tikz/above left/.code={\tikz@lib@place@handle@{##1}{south east}{-1}{1}{north west}{#2}},
      /tikz/above right/.code={\tikz@lib@place@handle@{##1}{south west}{1}{1}{north east}{#2}},
      /tikz/below left/.code={\tikz@lib@place@handle@{##1}{north east}{-1}{-1}{south west}{#2}},
      /tikz/below right/.code={\tikz@lib@place@handle@{##1}{north west}{1}{-1}{south east}{#2}}
    },
    rectangular/.style 2 args={
      /kD/every layout/.append style={/kD/layouts/rectangular={#1}{#2}},
      % TODO: how much of the following is necessary in layouts?
      /kD/diagrams/grid={#1}{#2},
      /kD/diagrams/metric={1 and 1}{1}
    },
    square/.style={
      /kD/every layout/.append style={/kD/layouts/square={#1}},
      /kD/diagrams/grid={#1}{#1},
      /kD/diagrams/metric={1 and 1}{1}
    },
    golden/.style={
      /kD/every layout/.append style={/kD/layouts/golden={#1}},
      /kD/diagrams/grid={#1}{0.618*#1},
      /kD/diagrams/metric={1 and 1}{1}
    },
    comb/.code args={#1step #2 angle #3}{
      % TODO: write better option parser
      \if\relax#1\pgfkeys{/kD/diagrams/horizontal comb=step #2 angle #3}
      \else\pgfkeys{/kD/diagrams/#1comb=step #2 angle #3}\fi
    },
    horizontal comb/.style args={step #1 angle #2}{
      /kD/every layout/.append style={/kD/layouts/horizontal comb=step #1 angle #2},
      /kD/diagrams/grid={#1*0.5}{#1*tan(#2)*0.5},
      /kD/diagrams/metric={2}{0.5}
    },
    vertical comb/.style args={step #1 angle #2}{
      /kD/every layout/.append style={/kD/layouts/vertical comb=step #1 angle #2},
      /kD/diagrams/grid={#1*tan(#2)*0.5}{#1*0.5},
      /kD/diagrams/metric={2}{0.5}
    },
    comb/.default=step 4.5em angle 60,
    rectangular/.default={6em}{4em},
    square/.default=4.5em,
    golden/.default=4.5em,
}

%==[ baseline centered rectangle shape ]========================================

% The math formula axis height is recovered and stored as a pgf function.

% NOTE: the LuaTeX version is needed just by ConTeXt
\pgfutil@ifluatex
  \directlua{tex.enableprimitives('kD', {'Umathaxis'})}
  \pgfmathdeclarefunction{kD_math_formula_axis_height}{0}{%
    \begingroup%
      $\relax$% update fontdimens
      % See TeX by Topic §23.5 for details.
      \pgfmathreturn\the\kDUmathaxis\textstyle%
    \endgroup}
\else% if using (pdf)tex
  \pgfmathdeclarefunction{kD_math_formula_axis_height}{0}{%
    \begingroup%
      $\relax$% update fontdimens
      % See TeX by Topic §23.5 for details.
      \pgfmathreturn\the\fontdimen22\textfont2%
    \endgroup}
\fi

\pgfqkeys{/kD/baseline centered rectangle}{
  center raise/.initial=kD_math_formula_axis_height
}

% Then the shape is defined by inheritance.

\pgfdeclareshape{kD baseline centered rectangle} {
  % Inherit the rectangle shape.
  \inheritsavedanchors[from={rectangle}]
  \inheritanchor[from={rectangle}]{base}
  \inheritanchor[from={rectangle}]{north}
  \inheritanchor[from={rectangle}]{south}
  \inheritanchor[from={rectangle}]{base west}
  \inheritanchor[from={rectangle}]{north west}
  \inheritanchor[from={rectangle}]{south west}
  \inheritanchor[from={rectangle}]{base east}
  \inheritanchor[from={rectangle}]{north east}
  \inheritanchor[from={rectangle}]{south east}
  \inheritanchor[from={rectangle}]{mid}
  \inheritanchor[from={rectangle}]{mid west}
  \inheritanchor[from={rectangle}]{mid east}
  \inheritbackgroundpath[from={rectangle}]
  % Redefine west, center and east anchors
  % setting their y coordinates to center raise.
  \anchor{center}{\pgf@anchor@rectangle@center\pgfmathsetlength\pgf@y%
    {\pgfkeysvalueof{/kD/baseline centered rectangle/center raise}}}
  \anchor{west}{\pgf@anchor@rectangle@west\pgfmathsetlength\pgf@y%
    {\pgfkeysvalueof{/kD/baseline centered rectangle/center raise}}}
  \anchor{east}{\pgf@anchor@rectangle@east\pgfmathsetlength\pgf@y%
    {\pgfkeysvalueof{/kD/baseline centered rectangle/center raise}}}
  % Save the original anchors as alternate "real" versions.
  \anchor{real center}{\pgf@anchor@rectangle@center}
  \anchor{real west}{\pgf@anchor@rectangle@west}
  \anchor{real east}{\pgf@anchor@rectangle@east}
  % Redefine the border anchor calculation.
  \anchorborder{%
    % (x,y) = target
    % let tempdima = center raise
    \pgfmathsetlength\pgfutil@tempdima%
      {\pgfkeysvalueof{/kD/baseline centered rectangle/center raise}}%
    % let b = (x,y) = target
    \pgf@xb=\pgf@x%
    \pgf@yb=\pgf@y%
    % let (x,y) = south west
    \southwest%
    % let a = (x,y) = south west
    \pgf@xa=\pgf@x%
    \pgf@ya=\pgf@y%
    % let (x,y) = north east
    \northeast%
    % let (x,y) = (x,y) - a = north east - south west = (width, height)
    \advance\pgf@x by-\pgf@xa%
    \advance\pgf@y by-\pgf@ya%
    % let c = (x,y)/2 = (width, height)/2 = (width/2, height/2)
    \pgf@xc=.5\pgf@x%
    \pgf@yc=.5\pgf@y%
    % let a = a + c = south west + (width/2, height/2) = center
    \advance\pgf@xa by\pgf@xc%
    \advance\pgf@ya by\pgf@yc%
    % if by = target y > 0
    \ifdim\pgf@yb>0pt%
      % let (x,y) = north east
      \northeast%
      % let cy = y = north east y
      \pgf@yc=\pgf@y%
      % let cy = cy - center raise = north east y - center raise
      \advance\pgf@yc by-\pgfutil@tempdima%
    \else%
      % let (x,y) = south west
      \southwest%
      % let cy = y = - south west y
      \pgf@yc=-\pgf@y%
      % let cy = cy + center raise = - south west y + center raise
      \advance\pgf@yc by\pgfutil@tempdima%
    \fi
    \edef\pgf@marshal{%
      % calculate the intersection of the half line from the origin
      \noexpand\pgfpointborderrectangle
      % passing through target
      {\noexpand\pgfqpoint{\the\pgf@xb}{\the\pgf@yb}}
      % and the rectangle centered on the origin
      % whose upper right corner is
      % (width/2, +north east y - center raise) if target y > 0
      % (width/2, -south west y + center raise) if target y < 0
      {\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@yc}}%
    }%
    % let (x,y) = the intersection
    \pgf@process{\pgf@marshal}%
    % let x = x + ax = width/2 + center x
    \advance\pgf@x by\pgf@xa%
    % let y = y + tempdima = ±(ne/sw y - center raise) + center raise
    \advance\pgf@y by\pgfutil@tempdima%
    % that is, y = + north east y                    if target y > 0
    %          y = - south west y + 2 * center raise if target y < 0
    %
    % NOTE: in essence, we're just compensating for the redefinition
    % of ne/sw anchors that shifted them by cr below the real center.
    %                ┏━━━━━━┯━━━━━━┓  ╮╮              
    %                ┃      │      ┃  ││ + ney - cr   
    %            ╭╭  ┠──────┼──────┨ ╮│╯               y > 0
    % - swy + cr │╰╭ ┣━━━━━━┿━━━━━━┫ ╯╯ ┈┈┈┈┈┈┈┈┈┈┈┈┈┈┈┈┈┈┈┈┈
    %            ╰ ╰ ┗━━━━━━┷━━━━━━┛                   y < 0
  }%
}%

%==[ training wheels ]==========================================================

% This key is meant for visual assistance with the node labeling automation.

\pgfqkeys{/kD}{
  training wheels label/.style={
    /tikz/.cd,
    inner sep=0sp,
    font=\ttfamily\bfseries\tiny,
    line width=1pt,
    draw=violet,
    fill=violet,
    text=white,
    overlay,
    label anchor/.style={tikz@label@post/.append style={anchor=##1}},
    label anchor=north east,
    label position=south east
  },
  training wheels pinner/.style={
    /tikz/draw=violet,
    /tikz/line width=1sp,
    /tikz/label={[/kD/training wheels label]:#1},
  },
  training wheels/.style={/bapto/output/.forward to=/kD/training wheels pinner}
}


==> tikzlibrarykodi.mitra.code.tex <==
% μήτρα • (mítra)
%   1. womb
%   2. matrix
%   3. mold

% Mitra is an alternative parsing mechanism for TiKz matrices of nodes.
% It couples with ozos to ensure the node contents  always pass through the TikZ key.

\usetikzlibrary{matrix}
\usetikzlibrary{kodi.koinos}

%==[ TikZ/pgf layer ]===========================================================

\pgfkeys{
  /mitra/every node/.style={},
  /mitra/every matrix/.style={
    /tikz/matrix,
    /tikz/cells={
      /tikz/anchor=base
    }
  },
  % NOTE: the alias key *cannot* be put along with global node styles
  %   because of execution order.
  /mitra/matrix coordinates alias/.style={
    /tikz/alias=\tikzmatrixname-\the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn
  }
}

%==[ main macro ]===============================================================

\def\kDMitra
  {\kDMitraFetchMatrixThen
  {\kDMitraParseMatrixTableThen
   \kDMitraOutput}}

% General purpose scratch register.
\newtoks\kDMitraTmpTok

%==[ fetching routine ]=========================================================

% I use the general one implemented by koinos.
\let\kDMitraFetchMatrixThen\kDFetchOptAndGrpThen

%==[ parsing routine: /table ]==================================================

\newtoks\kDMitraMatOutTok

\def\kDMitraParseMatrixTableThen#1{%
  \kDMitraMatOutTok={}%
  \expandafter\kDMitraParseTable\the\kDGrpTok\kD
  #1}

\def\kDMitraParseTable
  {\kDMitraParseAllRowsThen\relax}

\def\kDMitraParseAllRowsThen#1{%
  \def\kDExit{#1}%
  \kDIfNextHardCh\kD
    {\expandafter\kDExit\kDGobbleHardTok}%
    {\kDMitraParseOneRowThen{\kDMitraParseAllRowsThen{#1}}}}

%==[ parsing routine: /table/row ]==============================================

\def\kDMitraParseOneRowThen#1%
  {\kDMitraMarkRowEndBefore
  {\kDMitraParseAllColsThen
  {\kDMitraParseRowEndThen
  {#1}}}}

\kDStoreCatcodeOf &
\ifConTeXt\catcode`&=12\else\catcode`&=4\fi
\def\kDMitraMarkRowEndBefore#1#2\\{#1#2&\kD\\}
\kDRestoreCatcodeOf &

\def\kDMitraParseAllColsThen#1{%
  \def\kDExit{#1}%
  \kDIfNextHardCh\kD
    {\expandafter\kDExit\kDGobbleHardTok}%
    {\kDMitraParseOneColThen{\kDMitraParseAllColsThen{#1}}}}

\def\kDMitraParseRowEndThen#1%
  {\kDMitraFetchRowEndThen
  {\kDMitraPrintRowEndThen
  {#1}}}

\def\kDMitraFetchRowEndThen#1\\{\kDMitraMaybeFetchRowOptionsThen{#1}}

\newtoks\kDMitraRowOptTok

\def\kDMitraPrintRowEndThen#1{%
  \edef\kDAct{\noexpand\kDMitraTmpTok={\noexpand\\\the\kDMitraRowOptTok}}%
  \kDAct
  \kDAppend\kDMitraTmpTok\kDMitraMatOutTok
  #1}

\def\kDMitraMaybeFetchRowOptionsThen#1{%
  \kDMitraRowOptTok={}%
  \kDIfNextHardCh[%
    {\kDMitraFetchRowOptionsThen{#1}}%
    {#1}}

\def\kDMitraFetchRowOptionsThen#1[#2]{\kDMitraRowOptTok={[#2]}#1}

%==[ parsing routine: /table/row/column ]=======================================

\def\kDMitraParseOneColThen#1%
  {\kDMitraParseCellThen
  {\kDMitraParseColEndThen
  {#1}}}

\def\kDMitraParseColEndThen#1%
  {\kDMitraMaybeFetchColOptionsThen
  {\kDMitraMaybePrintColEndThen
  {#1}}}

\newtoks\kDMitraColOptTok

\def\kDMitraMaybeFetchColOptionsThen#1{%
  \kDMitraColOptTok={}%
  \kDIfNextHardCh[%
    {\kDMitraFetchColOptionsThen{#1}}%
    {#1}}

\def\kDMitraFetchColOptionsThen#1[#2]{\kDMitraColOptTok={[#2]}#1}

\def\kDMitraMaybePrintColEndThen#1{%
  \kDIfNextHardCh\kD
    {#1}%
    {% NOTE: we use \pgfmatrixnextcell instead of & to avoid catcode juggling
      \edef\kDAct{\noexpand\kDMitraTmpTok={\noexpand\pgfmatrixnextcell\the\kDMitraColOptTok}}%
      \kDAct
      \kDAppend\kDMitraTmpTok\kDMitraMatOutTok
      #1%
    }}

%==[ parsing routine: /table/row/column/cell ]==================================

\def\kDMitraParseCellThen#1%
  {\kDMitraMaybeFetchCellOptionsThen
  {\kDMitraFetchCellContentThen
  {\kDMitraPrintCellThen
  {#1}}}}

\newtoks\kDMitraCelOptTok

\def\kDMitraMaybeFetchCellOptionsThen#1{%
  \kDMitraCelOptTok={}%
  \kDIfNextHardCh|%
    {\kDMitraFetchCellOptionsThen{#1}}
    {#1}}

\def\kDMitraFetchCellOptionsThen#1|#2|{\kDMitraCelOptTok={#2}#1}

\newtoks\kDMitraCelCntTok

\kDStoreCatcodeOf &
\ifConTeXt\catcode`&=12\else\catcode`&=4\fi
\def\kDMitraFetchCellContentThen#1#2&{%
  \kDMitraCelCntTok={#2}%
  \kDTrimLeadingSpace\kDMitraCelCntTok
  \kDTrimTrailingSpace\kDMitraCelCntTok
  #1}
\kDRestoreCatcodeOf &

\def\kDMitraMaybeDoCellThen#1{%
  \kDIfNextHardCh\kD
    {#1}%
    {\kDMitraParseOneColThen{#1}}}

\def\kDMitraPrintCellThen#1{%
  \edef\kDAct{%
    \noexpand\kDMitraTmpTok={%
      \noexpand\node
        [/mitra/every node]
        \the\kDMitraCelOptTok
        [node contents={\the\kDMitraCelCntTok},/mitra/matrix coordinates alias];
      \kDMitraMaybeDumpCell}}%
  \kDAct
  \kDAppend\kDMitraTmpTok\kDMitraMatOutTok
  #1}

%==[ dumping routine ]==========================================================

\def\kDMitraMaybeDumpCell{\noexpand\pgfextra{%
  \noexpand\kDDump{'\noexpand\the\noexpand\pgfmatrixcurrentrow-\noexpand\the\noexpand\pgfmatrixcurrentcolumn':}%
  \noexpand\kDDump{\space\space options: '\the\kDMitraCelOptTok'}%
  \noexpand\kDDump{\space\space content: '\the\kDMitraCelCntTok'}}}

%==[ output routine ]===========================================================

\def\kDMitraOutput{%
  \edef\kDAct{%
    \noexpand\kDMitraTmpTok={%
      \noexpand\matrix
        [/mitra/every matrix]%
        \the\kDOptTok
        {\the\kDMitraMatOutTok};}}%
  \kDAct
  \the\kDMitraTmpTok}


==> tikzlibrarykodi.ozos.code.tex <==
% όζος • (ózos)
%   1. node
%   2. nodule
%   3. gnarl

% Ozos is an alternative parsing mechanism for TiKz nodes.
% It implements the following transformation
%   \kDOzos ... {CONTENTS};  --->  \node ... [node contents={CONTENTS}];
% to ensure the node contents always pass through the TikZ key.

\usetikzlibrary{kodi.koinos}

%==[ TikZ/pgf layer ]===========================================================

\pgfkeys{/ozos/every node/.style={}}

%==[ main macro ]===============================================================

\def\kDOzos%
  {\kDOzosFetchThen
  {\kDOzosMaybeDumpThen
   \kDOzosOutput}}

%==[ fetching routine ]=========================================================

% I use the general one implemented by koinos.
\let\kDOzosFetchThen\kDFetchOptAndGrpThen

%==[ parsing routine ]==========================================================

% Trivially solved by fetching.

%==[ dumping routine ]==========================================================

\def\kDOzosMaybeDumpThen#1{%
  \kDDump{options: '\the\kDOptTok'}%
  \kDDump{content: '\the\kDGrpTok'}%
  #1}

%==[ output routine ]===========================================================

\def\kDOzosOutput{
  \edef\kDAct{
    \noexpand\node
      [/ozos/every node]
      \the\kDOptTok
      [/tikz/node contents={\the\kDGrpTok}];
  }
  \kDAct
}


==> tikzlibrarykodi.ramma.code.tex <==
% ράμμα • (rámma)
%   1. suture
%   2. catgut
%   3. stitch

% Ramma ties together the lower level libraries to define
% the user level functionality. NOTE: strictly no aesthetics, see mandyas.

\usetikzlibrary[kodi.bapto]
\usetikzlibrary[kodi.ektropi]
\usetikzlibrary[kodi.katharizo]
\usetikzlibrary[kodi.koinos]
\usetikzlibrary[kodi.ozos]
\usetikzlibrary[kodi.mitra]
\usetikzlibrary[kodi.velos]

%==[ core concept ]=============================================================

\pgfqkeys{/kD}{% TODO: is this the best scope to put the key into?
  self naming/.style={
    /tikz/node contents/.forward to=/bapto/input,
    /bapto/trigger/.forward to=/katharizo/input,
    /katharizo/output/.forward to=/bapto/dispatcher
  }
}

%==[ baseline setup ]===========================================================

% Some mischief with handlers and baseline math/labeling functionality.

\pgfqkeys{/kD}{
  .search also=/bapto,
  .search also=/katharizo,
  every thing/.style={
    /ektropi/restore,
    /ektropi/add=/kD,
    /ektropi/add=/bapto,
    /ektropi/add=/katharizo
  },
  every diagram/.style={% NOTE: restore hopefully unnecessary
    /kD/every thing,
    /ektropi/add=/kD/diagrams
  },
  every layout/.style={% NOTE: restore actually unnecessary
    /kD/every thing,
    /ektropi/add=/kD/layouts,
    /mitra/every node/.append style={/kD/every object}
  },
  every object/.style={% NOTE: needed when inside matrices
    /kD/every thing,
    /ektropi/add=/kD/objects,
    execute at begin node=$,%
    execute at end node=$,%
    /kD/self naming
  },
  every arrow/.style={% NOTE: restore unnecessary
    /kD/every thing,
    /ektropi/add=/kD/arrows
  },
  every label/.style={% NOTE: restore needed because inside edge
    /kD/every thing,
    /ektropi/add=/kD/labels,
    execute at begin node=$,%
    execute at end node=$,%
    /kD/self naming
  }
}

% The user level keys are bound to the underlying parsers.

\pgfkeys{
  /mitra/every matrix/.append style=/kD/every layout,
  /ozos/every node/.append style=/kD/every object,
  /velos/every path/.append style={
    /tikz/every edge/.append style=/kD/every arrow,
    /tikz/every edge quotes/.append style=/kD/every label
  }
}

% I merge the macro syntax for objects and matrices. Convenient!

\newif\ifkDRammaObjIsMatrix

\def\kDRammaObjDecideWhetherIsMatrixThen#1{%
  \def\kDRammaObjDWIM{\kDRammaObjDWIMSightThen{\kDRammaObjDWIMGobThen{#1}}}%
  \expandafter\kDRammaObjDWIM\the\kDGrpTok\\\kD}

\def\kDRammaObjDWIMSightThen#1#2\\%
  {\kDIfNextHardCh\kD
    {\kDRammaObjIsMatrixfalse#1}%
    {\kDRammaObjIsMatrixtrue#1}}

\def\kDRammaObjDWIMGobThen#1#2\kD{#1}

\def\kDRammaObjOutput
  {\ifkDRammaObjIsMatrix
    \kDMitraParseMatrixTableThen\kDMitraOutput\else
    \kDOzosOutput\fi}

\def\kDRammaObj
  {\kDFetchOptAndGrpThen
  {\kDRammaObjDecideWhetherIsMatrixThen
   \kDRammaObjOutput}}

% Just an identity.
\let\kDRammaMor\kDVelos

%==[ TikZ/pgf layer ]===========================================================

% I envelope the koDi main macros in a simple key for maximal flexibility.

\tikzset{
  kodi/.code={%
    \ifConTeXt\catcode`\|=12\fi% TODO: is it sufficient? investigate
    \let\obj\kDRammaObj
    \let\mor\kDRammaMor
  },
  kodi/.append style={/kD/every diagram}
}

%==[ main macro ]===============================================================

\def\kDRamma
  {\kDRammaMaybeFetchOptionsThen
   \kDRammaOutput}

\let\kDRammaOpen\kDRamma
\let\kDRammaShut\endtikzpicture

%==[ fetching routine ]=========================================================

\newtoks\kDRammaOptTok
\newtoks\kDRammaTmpTok

\def\kDRammaMaybeFetchOptionsThen#1{%
  \kDRammaOptTok={}%
  \kDIfNextHardCh[%
    {\kDRammaFetchOptionsThen{#1}}%
    {#1}}

\def\kDRammaFetchOptionsThen#1[#2]{\kDRammaOptTok={#2}#1}

%==[ output routine ]===========================================================

\def\kDRammaOutput{%
  \edef\kDAct{%
    \noexpand\kDRammaTmpTok={%
      \noexpand\tikzpicture[kodi, \the\kDRammaOptTok]}}%
  \kDAct
  \the\kDRammaTmpTok}


==> tikzlibrarykodi.velos.code.tex <==
% βέλος • (vélos)
%   1. arrow
%   2. dart
%   3. shaft

% Velos is a parsing mechanism for arrow chains.

\usetikzlibrary{kodi.koinos}

%==[ TikZ/pgf layer ]===========================================================

\pgfkeys{
  % NOTE: there might be some way to work w/ quotes library, but it's safer and
  %   easier to just have a custom handler mounted in the maximally local scope
  %   and avoid any conflict a priori.
  /velos/install quote handler/.style={
    /handlers/first char syntax=true,
    /handlers/first char syntax/the character "/.initial=\kDVelosQuoteHandler
    % node quotes mean={node contents={#1}},
    % edge quotes mean={node contents={#1}}
  },
  /velos/every path/.style={
    /velos/install quote handler
  }
}

\def\kDVelosQuoteHandler#1%
  {\pgfkeysalso{/tikz/node contents/.expand once={\kDVelosUnquote#1}}}

\def\kDVelosUnquote"#1"{#1}

%==[ global options ]===========================================================

\newtoks\kDVelosTemp

\newtoks\kDVelosGlobalLabelOptions
\newtoks\kDVelosGlobalEdgeOptions

\newif\ifkDVelosGOAfterColon

\def\kDVelosFetchGlobalOptionsThen#1{%
  \kDVelosGOAfterColonfalse
  \kDVelosGlobalLabelOptions={}%
  \kDVelosGlobalEdgeOptions={}%
  \kDVelosGOMaybeFetchThen{\kDVelosGOThinkThen{#1}}}

\def\kDVelosGOMaybeFetchThen#1{%
  \kDVelosTemp={}%
  \kDIfNextHardCh[%
    {\kDVelosGOFetchThen{#1}}%
    {#1}}

\def\kDVelosGOFetchThen#1[#2]{%
  \kDVelosTemp={#2}%
  #1}

\def\kDVelosGOThinkThen#1{%
  \def\kDVelosGOLoop{\kDVelosGOThinkThen{#1}}%
  \def\kDVelosGOBreak{#1}%
  \kDIfNextHardCh:%
    {%
      \kDVelosGOAfterColontrue
      \kDVelosGlobalLabelOptions\expandafter{\the\kDVelosTemp}%
      \expandafter\kDVelosGOMaybeFetchThen\expandafter\kDVelosGOLoop\kDGobbleHardTok
    }{%
      \ifkDVelosGOAfterColon
        \kDVelosGlobalEdgeOptions\expandafter{\the\kDVelosTemp}\else
        \kDVelosGlobalLabelOptions\expandafter{\the\kDVelosTemp}\fi
      \kDVelosGOBreak
    }}

%==[ first edge ]===============================================================

\def\kDVelosDoFirstEdgeThen#1%
  {\kDVelosFetchFirstSourceThen
  {\kDVelosFetchFirstEdgeThen
  {\kDVelosDrawFetchedEdgeThen
  {#1}}}}

\newtoks\kDVelosSource
\newtoks\kDVelosCurFstSrc
\newtoks\kDVelosPrvFstSrc

\def\kDVelosFetchFirstSourceThen#1%
  {\kDIfNextHardCh(%
    {\kDVelosFFSBracketsThen{#1}}%
    {\kDVelosFFSTillOverThen{#1}}}

\def\kDVelosFFSBracketsThen#1(#2){%
  \kDVelosSource={#2}%
  \kDVelosCurFstSrc={#2}%
  #1}

\def\kDVelosFFSTillOverThen#1#2 {% <- mind the space!
  \kDVelosSource={#2}%
  \kDVelosCurFstSrc={#2}%
  #1}

\def\kDVelosFetchFirstEdgeThen#1%
  {\kDVelosFetchEdgeThen
  {\kDVelosFetchTargetThen
  {#1}}}

%==[ chained edges ]============================================================

\newtoks\kDVelosEdge

\def\kDVelosFetchEdgeThen#1{%
  \kDVelosEdge={}%
  \kDVelosFEThen{\kDVelosFEThinkThen{#1}}}

\def\kDVelosFEThen#1%
  {\kDIfNextHardCh[%
    {\kDVelosFEKeysListThen{#1}}%
    {\kDIfNextHardCh"%
      {\kDVelosFEEnquotedThen{#1}}%
      {\kDVelosFETillOverThen{#1}}}}

\newif\ifkDVelosTempIsKeysList

\def\kDVelosFEEnquotedThen#1"#2"{%
  \kDVelosTempIsKeysListfalse
  \kDVelosTemp={#2}%
  #1}

\def\kDVelosFEKeysListThen#1[#2]{%
  \kDVelosTempIsKeysListtrue
  \kDVelosTemp={#2}%
  #1}

\def\kDVelosFETillOverThen#1{%
  \kDVelosTempIsKeysListfalse
  \kDVelosTemp={}%
  \kDVelosFETOThen{#1}}

\def\kDVelosFETOThen#1%
  {\kDIfNextSoftCh\kDBlankSpace
    {#1}%
    {\kDIfNextHardCh:%
      {#1}
      {\kDVelosFEAppendThen{\kDVelosFETOThen{#1}}}}}

\def\kDVelosFEAppendThen#1#2{%
  \kDVelosTemp=\expandafter{\the\kDVelosTemp#2}%
  #1}

\def\kDVelosFEEdgePrepend#1{%
  \edef\Act{\noexpand\kDVelosEdge={#1,\the\kDVelosEdge}}%
  \Act}

\def\kDVelosFEEdgePrependNode#1%
  {\kDVelosFEEdgePrepend{edge node={node[every edge quotes][/velos/install quote handler,#1]}}}

\def\kDVelosFEThinkThen#1{%
  \def\kDVelosFELoop{\kDVelosFEThinkThen{#1}}%
  \def\kDVelosFEBreak{#1}%
  \kDIfNextHardCh[%
    {%
      \kDVelosFEEdgePrependNode{\the\kDVelosTemp}%
      \kDVelosFEThen\kDVelosFELoop
    }{%
      \kDIfNextHardCh:%
        {%
          \ifkDVelosTempIsKeysList
            \kDVelosFEEdgePrependNode{\the\kDVelosTemp}\else
            \kDVelosFEEdgePrependNode{"\the\kDVelosTemp"}\fi
          \expandafter\kDVelosFEThen\expandafter\kDVelosFELoop\kDGobbleHardTok
        }{%
          \kDVelosFEEdgePrepend{\the\kDVelosTemp}%
          \kDVelosFEBreak
        }%
    }}

%==[ target ]===================================================================

\newtoks\kDVelosTarget
\newtoks\kDVelosCurLstTar
\newtoks\kDVelosPrvLstTar

\def\kDVelosFetchTargetThen#1%
  {\kDIfNextHardCh(%
    {\kDVelosFTBracketsThen{#1}}%
    {\kDVelosFTTillOverThen{#1}}}

\def\kDVelosFTBracketsThen#1(#2){%
  \kDVelosTarget={#2}%
  \kDVelosCurLstTar={#2}%
  #1}

\def\kDVelosFTTillOverThen#1{%
  \kDVelosTarget={}%
  \kDVelosFTTOThen{#1}}

\def\kDVelosFTTOThen#1{%
  \def\kDVelosFTTOLoop%
    {\kDVelosFTTOThen{#1}}%
  \def\kDVelosFTTOExit{%
    \kDVelosCurLstTar\expandafter{\the\kDVelosTarget}%
    #1}%
  \kDIfNextSoftCh\kDBlankSpace
    {\kDVelosFTTOExit}%
    {\kDIfNextHardCh;%
      {\kDVelosFTTOExit}%
      {\kDVelosFTAppendThen\kDVelosFTTOLoop}}}

\def\kDVelosFTAppendThen#1#2{%
  \kDVelosTarget=\expandafter{\the\kDVelosTarget#2}%
  #1}

%==[ rendering/dereferencing ]==================================================

\def\kDVelosAlias{*}
\def\kDVelosSaila{+}

\newtoks\kDVelosDerefSrc
\newtoks\kDVelosDerefTar

\def\kDVelosDrawFetchedEdgeThen#1{
  \edef\cS{\the\kDVelosSource}%
  \kDVelosDerefSrc\expandafter{\the\kDVelosSource}%
  \ifx\cS\kDVelosAlias\kDVelosDerefSrc\expandafter{\the\kDVelosPrvFstSrc}\fi
  \ifx\cS\kDVelosSaila\kDVelosDerefSrc\expandafter{\the\kDVelosPrvLstTar}\fi
  \edef\cT{\the\kDVelosTarget}%
  \kDVelosDerefTar\expandafter{\the\kDVelosTarget}%
  \ifx\cT\kDVelosAlias\kDVelosDerefTar\expandafter{\the\kDVelosPrvLstTar}\fi
  \ifx\cT\kDVelosSaila\kDVelosDerefTar\expandafter{\the\kDVelosPrvFstSrc}\fi
  \edef\Act{%
    \noexpand\path
      [/velos/every path]%
      [%
        /tikz/every edge/.append style=%
          {\the\kDVelosGlobalEdgeOptions},%
        /tikz/every edge quotes/.append style=%
          {auto,\the\kDVelosGlobalLabelOptions},%
      ]%
      (\the\kDVelosDerefSrc)%
      edge[\the\kDVelosEdge]%
      (\the\kDVelosDerefTar);}%
  \Act%
  #1}

%==[ high level ]===============================================================

\def\kDVelos%
  {\kDVelosFetchGlobalOptionsThen
  {\kDVelosDoFirstEdgeThen
   \kDVelosMaybeChainEdge}}

\def\kDVelosMaybeChainEdge{%
  \kDIfNextHardCh;%
    {%
    \edef\cS{\the\kDVelosCurFstSrc}%
    \ifx\cS\kDVelosAlias
      \kDVelosCurFstSrc\expandafter{\the\kDVelosPrvFstSrc}%
    \else\ifx\cS\kDVelosSaila
      \kDVelosCurFstSrc\expandafter{\the\kDVelosPrvLstTar}%
    \fi\fi
    \edef\cT{\the\kDVelosCurLstTar}%
    \ifx\cT\kDVelosAlias
      \kDVelosCurLstTar\expandafter{\the\kDVelosPrvLstTar}%
    \else\ifx\cT\kDVelosSaila
      \kDVelosCurLstTar\expandafter{\the\kDVelosPrvFstSrc}%
    \fi\fi
    \kDVelosPrvFstSrc\expandafter{\the\kDVelosCurFstSrc}%
    \kDVelosPrvLstTar\expandafter{\the\kDVelosCurLstTar}%
    }{%
      \kDVelosSource\expandafter{\the\kDVelosTarget}
      \kDVelosFetchEdgeThen
        {\kDVelosFetchTargetThen
        {\kDVelosDrawFetchedEdgeThen
         \kDVelosMaybeChainEdge}}%
    }}
